Generalizable autoregressive modeling of time series through functional narratives

Time series data are inherently functions of time, yet current transformers often learn time series by modeling them as mere concatenations of time periods, overlooking their functional properties. In this work, we propose a novel objective for transformers that learn time series by re-interpreting them as temporal functions. We build an alternative sequence of time series by constructing degradation operators of different intensity in the functional space, creating augmented variants of the original sample that are abstracted or simplified to different degrees. Based on the new set of generated sequence, we train an autoregressive transformer that progressively recovers the original sample from the most simplified variant. Analogous to the next word prediction task in languages that learns narratives by connecting different words, our autoregressive transformer aims to learn the Narratives of Time Series (NoTS) by connecting different functions in time. Theoretically, we justify the construction of the alternative sequence through its advantages in approximating functions. When learning time series data with transformers, constructing sequences of temporal functions allows for a broader class of approximable functions (e.g., differentiation) compared to sequences of time periods, leading to a 26\% performance improvement in synthetic feature regression experiments. Experimentally, we validate NoTS in 3 different tasks across 22 real-world datasets, where we show that NoTS significantly outperforms other pre-training methods by up to 6\%. Additionally, combining NoTS on top of existing transformer architectures can consistently boost the performance. Our results demonstrate the potential of NoTS as a general-purpose dynamic learner, offering a viable alternative for developing foundation models for time series analysis.

==> tables/ablation_table.tex <==

\begin{table}[h!]
  \begin{center}
    \caption{\footnotesize Ablation of training method. {\color{blue} If it is just one row, make it a figure?}
    }
    \label{tab:encoder-ablation}
      \begin{tabular}{c|c|c|c|c} 
       & Ours & Remove consistency term & Remove Autoregressive & Remove augmentations \\
      \hline
Results & & & & \\
    \end{tabular}
  \end{center}
\end{table}

==> tables/realworld_table.tex <==
\begin{table}[t!]
\addtolength{\tabcolsep}{-0.4em}
  \begin{center}
    \caption{\footnotesize In-context performance and data-specific tuning performance on real-world datasets.
    }
    \label{tab:synthetic}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c?cccc?cccccc} % <-- 
    &  \multicolumn{4}{c}{\textit{\large Prompt Tuning ($<1\%$ new params)}} & \multicolumn{6}{c}{\textit{\large Task-specific training and tuning}} \\
    % \hline
    \textbf{Classification} & \textbf{\ourslw} & Next-period & SimMTM & bioFAME & \textbf{\ourslw} & TimesNet & iTransformer & PatchTST & DLinear & \\
    \textbf{(14 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & \textbf{(Ours)} & \tiny{\cite{wu2022timesnet}} & \tiny{\cite{zhou2022fedformer}} & \tiny{\cite{zhou2021informer}} & \tiny{\cite{zhang2022less}} & \tiny{\cite{zeng2023transformers}} \\
        \thickhline
\footnotesize{UEA-subset} & 62.83 & 57.92 & 57.44 & 58.97 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
\footnotesize{UCR-subset} & 63.63 & 56.20 & 58.83 & 57.33 & & & & & & \\
\footnotesize{TFC} & & & & & & & & & & \\
    \hline
\footnotesize{\textbf{Avg.}} & & & & & & & & & & \\ 
    \\

    
\textbf{Imputation} & \textbf{\ourslw} & Next-Period & SimMTM & bioFAME & \textbf{\ourslw} & TimesNet & Stationary & Autoformer & iTransformer & DLinear \\
\textbf{(4 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & \textbf{(Ours)} & \tiny{\cite{wu2022timesnet}} & \tiny{\cite{}} & \tiny{\cite{}} & \tiny{\cite{}} & \tiny{\cite{zeng2023transformers}} \\
    \thickhline
\footnotesize{ETTm1} & 0.169 & 0.348 & 0.172 & 0.168 & 0.000 & 0.107 & 0.126 & 0.150 & 0.000 & 0.206 \\
\footnotesize{ETTm2} & 0.102 & 0.179 & 0.122 & 0.120 & & 0.088 & 0.099 & 0.105 & & 0.208 \\
\footnotesize{ETTh1} & 0.259 & 0.438 & 0.271 & 0.262 & & 0.187 & 0.201 & 0.214 & & 0.306 \\
\footnotesize{ETTh2} & 0.191 & 0.266 & 0.196 & 0.192 & & 0.146 & 0.152 & 0.156 & & 0.259 \\
    \hline
\footnotesize{\textbf{Avg.}} & \textbf{0.180} & 0.308 & 0.190 & 0.186 & & 0.132 & 0.145 & 0.156 & & 0.245 \\ 
    \\

\textbf{Ch-wise Imp.} & \textbf{\ourslw} & Next-Period & SimMTM & bioFAME & \textbf{\ourslw} & TimesNet & Stationary & Autoformer & iTransformer & DLinear \\
\textbf{(4 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & \textbf{(Ours)} & \tiny{\cite{wu2022timesnet}} & \tiny{\cite{}} & \tiny{\cite{}} & \tiny{\cite{}} & \tiny{\cite{zeng2023transformers}} \\
    \thickhline
\footnotesize{ETTm1} & 0.182 & 0.357 & 0.187 & 0.184 & 0.132 & 0.127 & 0.000 & 0.000 & 0.000 & 0.000 \\
\footnotesize{ETTm2} & 0.127 & 0.182 & 0.128 & 0.126 & 0.094 & 
0.116 & & & & \\
\footnotesize{ETTh1} & 0.273 & 0.453 & 0.301 & 0.297 & 0.201 & 0.240 & & & & \\
\footnotesize{ETTh2} & 0.193 & 0.267 & 0.199 & 0.196 & 0.163 & 0.216 & & & & \\
    \hline
\footnotesize{\textbf{Avg.}} & \textbf{0.194} & 0.315 & 0.204 & 0.200 & \textbf{0.147} & 0.175 & & & & \\ 
    \\
    
\textbf{Anom. Det.} & \textbf{\ourslw} & Next-Period & SimMTM & bioFAME & \textbf{\ourslw} & TimesNet & FedFormer & Informer & LightTS & DLinear \\
\textbf{(4 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & \textbf{(Ours)} & \tiny{\cite{wu2022timesnet}} & \tiny{\cite{zhou2022fedformer}} & \tiny{\cite{zhou2021informer}} & \tiny{\cite{zhang2022less}} & \tiny{\cite{zeng2023transformers}} \\
    \thickhline
\footnotesize{SMD} & 82.92 & 81.00 & 81.99 & 83.87 & 87.13 & 85.12 & 85.08 & 81.65 & 82.53 & 77.10 \\
\footnotesize{MSL} & 83.53 & 82.50 & 81.90 & 82.56 & 85.02 & 84.18 & 78.57 & 84.06 & 78.95 & 84.88 \\
% \footnotesize{SMAP} & & & & & & & & & & \\
\footnotesize{SWaT} & 93.26 & 87.46 & 85.69 & 88.01
 & 93.26 & 92.10 & 93.19 & 81.43 & 93.33 & 87.52 \\
\footnotesize{PSM} & 96.15 & 96.56 & 95.06 & 95.97 & 97.38 & 95.21 & 97.23 & 77.10 & 97.15 & 93.55 \\
    \hline
\footnotesize{\textbf{Avg.}} & \textbf{88.97} & 86.88 & 86.16 & 87.60 & \textbf{90.70} & 89.15 & 88.52 & 81.06 & 87.99 & 85.76
    
%\textbf{Forecasting} & \textbf{\ours} & Next-Period & SimMTM & bioFAME & \textbf{\ours} & \textbf{\ours~(Aug.)} & TimesNet & iTransformer & PatchTST & DLinear \\
%    \thickhline
%\footnotesize{ETTm1} & 00.00 & 00.00 & 00.00 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
%\footnotesize{ETTm2} & & & & & & & & & & \\
%\footnotesize{ETTh1} & & & & & & & & & & \\
%\footnotesize{ETTh2} & & & & & & & & & & \\
%    \hline
%\footnotesize{\textbf{Avg.}} & & & & & & & & & & \\
    % \hline
    \end{tabular}}
  \end{center}
\end{table}


==> tables/realworld_table_v2.tex <==
\begin{table}[t!]
\addtolength{\tabcolsep}{-0.4em}
  \begin{center}
    \caption{\footnotesize In-context performance and data-specific tuning performance on real-world datasets.
    }
    \label{tab:synthetic}
\resizebox{\linewidth}{!}{%
\begin{tabular}{c?cccc?ccccc} % <-- 
    &  \multicolumn{4}{c}{\textit{\large Prompt Tuning ($<1\%$ new params)}} & \multicolumn{5}{c}{\textit{\large Task-specific training and tuning}} \\
    % \hline
    \textbf{Classification} & \textbf{\ourslw} & Next-period & SimMTM & bioFAME & PatchTST & +\textbf{\ours} & iTransformer & +\textbf{\ours} & \textbf{\ourslw}  \\
    \textbf{(14 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & [cite] & \textbf{(Ours)} & [cite] & \textbf{(Ours)} & \textbf{(Ours)} \\
        \thickhline
\footnotesize{UEA-subset} & 62.83 & 57.92 & 57.44 & 58.97 & 0.000 & 0.000 & 0.000 & 0.000 \\
\footnotesize{UCR-subset} & 63.63 & 56.20 & 58.83 & 57.33 & & & & & \\
\footnotesize{TFC} & & & & & & & & & \\
    \hline
\footnotesize{\textbf{Avg.}} & & & & & & & & & \\ 
    \\

    \multicolumn{10}{c}{wrong number note edit soon} \\
\textbf{Imputation} & \textbf{\ourslw} & Next-Period & SimMTM & bioFAME & PatchTST & +\textbf{\ours} & iTransformer & +\textbf{\ours} & \textbf{\ourslw} \\
\textbf{(4 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & [cite] & \textbf{(Ours)} & [cite] & \textbf{(Ours)} & \textbf{(Ours)} \\
    \thickhline
\footnotesize{ETTm1} & 0.169 & 0.348 & 0.172 & 0.168 & 0.000 & 0.107 & 0.126 & 0.150 & \\
\footnotesize{ETTm2} & 0.102 & 0.179 & 0.122 & 0.120 & & 0.088 & 0.099 & 0.105 & \\
\footnotesize{ETTh1} & 0.259 & 0.438 & 0.271 & 0.262 & & 0.187 & 0.201 & 0.214 & \\
\footnotesize{ETTh2} & 0.191 & 0.266 & 0.196 & 0.192 & & 0.146 & 0.152 & 0.156 & \\
    \hline
\footnotesize{\textbf{Avg.}} & \textbf{0.180} & 0.308 & 0.190 & 0.186 & & 0.132 & 0.145 & 0.156 & \\ 
    \\

    \multicolumn{10}{c}{wrong number note edit soon} \\
\textbf{Ch-wise Imp.} & \textbf{\ourslw} & Next-Period & SimMTM & bioFAME & PatchTST & +\textbf{\ours} & iTransformer & +\textbf{\ours} & \textbf{\ourslw} \\
\textbf{(4 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & [cite] & \textbf{(Ours)} & [cite] & \textbf{(Ours)} & \textbf{(Ours)} \\
    \thickhline
\footnotesize{ETTm1} & 0.182 & 0.357 & 0.187 & 0.184 & 0.132 & 0.127 & 0.000 & 0.000 & 0.000 \\
\footnotesize{ETTm2} & 0.127 & 0.182 & 0.128 & 0.126 & 0.094 & 
0.116 & & & \\
\footnotesize{ETTh1} & 0.273 & 0.453 & 0.301 & 0.297 & 0.201 & 0.240 & & & \\
\footnotesize{ETTh2} & 0.193 & 0.267 & 0.199 & 0.196 & 0.163 & 0.216 & & & \\
    \hline
\footnotesize{\textbf{Avg.}} & \textbf{0.194} & 0.315 & 0.204 & 0.200 & \textbf{0.147} & 0.175 & & & \\ 
    \\

        \multicolumn{10}{c}{wrong number note edit soon} \\
\textbf{Anom. Det.} & \textbf{\ourslw} & Next-Period & SimMTM & bioFAME & PatchTST & +\textbf{\ours} & iTransformer & +\textbf{\ours} & \textbf{\ourslw} \\
\textbf{(4 datasets)} & \textbf{(Ours)} & Prediction & \tiny{\cite{dong2024simmtm}} & \tiny{\cite{liu2023frequency}} & [cite] & \textbf{(Ours)} & [cite] & \textbf{(Ours)} & \textbf{(Ours)} \\
    \thickhline
\footnotesize{SMD} & 82.92 & 81.00 & 81.99 & 83.87 & 87.13 & 85.12 & 85.08 & 81.65 & 82.53 \\
\footnotesize{MSL} & 83.53 & 82.50 & 81.90 & 82.56 & 85.02 & 84.18 & 78.57 & 84.06 & 78.95 \\
% \footnotesize{SMAP} & & & & & & & & & & \\
\footnotesize{SWaT} & 93.26 & 87.46 & 85.69 & 88.01
 & 93.26 & 92.10 & 93.19 & 81.43 & 93.33 \\
\footnotesize{PSM} & 96.15 & 96.56 & 95.06 & 95.97 & 97.38 & 95.21 & 97.23 & 77.10 & 97.15 \\
    \hline
\footnotesize{\textbf{Avg.}} & \textbf{88.97} & 86.88 & 86.16 & 87.60 & \textbf{90.70} & 89.15 & 88.52 & 81.06 & 87.99
    
%\textbf{Forecasting} & \textbf{\ours} & Next-Period & SimMTM & bioFAME & \textbf{\ours} & \textbf{\ours~(Aug.)} & TimesNet & iTransformer & PatchTST & DLinear \\
%    \thickhline
%\footnotesize{ETTm1} & 00.00 & 00.00 & 00.00 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 & 0.000 \\
%\footnotesize{ETTm2} & & & & & & & & & & \\
%\footnotesize{ETTh1} & & & & & & & & & & \\
%\footnotesize{ETTh2} & & & & & & & & & & \\
%    \hline
%\footnotesize{\textbf{Avg.}} & & & & & & & & & & \\
    % \hline
    \end{tabular}}
  \end{center}
\end{table}


==> tables/task_table.tex <==

\begin{table}[t!]
  \begin{center}
    \caption{\footnotesize Summary of experiments.
    }
    \label{tab:tasks}
      \begin{tabular}{c|c|c|c} 
      Tasks & Datasets & Metrics & Notes \\
      \hline
\multirow{2}{*}{Classification} 
    & Univariate (UCR, xx subset) & \multirow{2}{*}{Accuracy} & \\
    & Multivariants (UEA, xx subset) & & \\
Anomaly Detection & & & \\
Imputation  & & & \\
      \hline
    \end{tabular}
  \end{center}
\end{table}

==> text/app_wenrui_former.tex <==

\subsection{Bio-features details}

\todo[]{Wenrui: Organize and put your content in this section gradually.}

Consider $\mathbf{x} \in \mathbb{R}^{C \times T}$, where $C$ is the total amount of channels, and $T$ is the total amount of timestamps. We consider each entry as $x_{i, j}$, which refers to the $i$-th channel $j$-th timestamp value.

For simplicity, we also denote $x_i \in \mathbb{R}^{T}$ as the $i$-th channel of timeseries; and $x_j \in \mathbb{R}^{C}$ as the $j$-th timestamps of all channel activities.

\subsubsection{Frequency-related}

\paragraph{band power (BP)} One first take Fourier transform of the signal following:
\[
 XXXX
\]
and then perform summation or integral of the segments of frequencies:
\[
    XXXX
\]
In the meantime, we also compute Log Energy Entropy (LEE) to be the energy measure of the spectrum power.

sla


\paragraph{Entropy} 
Given a discrete random variable \(X\) with probability distribution \(P = \{p_1, p_2, \ldots, p_n\}\), the Rényi entropy of order \(\alpha\) (\(\alpha > 0\), \(\alpha \neq 1\)) is defined as:
\[
H_{\alpha}(X) = \frac{1}{1 - \alpha} \log \left( \sum_{i=1}^{n} p_i^{\alpha} \right)
\]
where \(H_{\alpha}(X)\) is the Rényi entropy of \(X\) for a given \(\alpha\), and \(\log\) denotes the logarithm, which can be taken to any base, commonly base 2 for information theoretic applications.
For a discrete random variable \(X\) with a probability distribution \(P = \{p_1, p_2, \ldots, p_n\}\), the Tsallis entropy of order \(q\) is defined as:
\[
S_q(P) = \frac{1}{q-1} \left(1 - \sum_{i=1}^{n} p_i^q \right)
\]
where \(S_q(P)\) is the Tsallis entropy for a given entropic index \(q\). Unlike the Rényi entropy, Tsallis entropy is non-extensive for \(q \neq 1\), meaning that the total entropy of a system is not simply the sum of its parts' entropies for non-additive systems.


\subsubsection{Power-related} In this paragraph, we consider properties that are related to the overall power or variation of the timeseries. We note that many bio-features have redundant or similar definitions, and our selection of features covers a wide rang of them with simple manipulations.

% Root Mean Square (RMS), Mean Absolute Value (MAV), Waveform Length (WL), Zero Crossing (ZC), Willison Amplitude (WAMP): These traditional EMG features offer various perspectives on the signal's power, average activation level, complexity, frequency content, and activation spikes. They are foundational in EMG analysis for assessing muscle performance, fatigue, and coordination.
\paragraph{Radio spectrum}
This is also called the power band ratio which is the power in different frequency bands for each channel, each window. The frequency band considered here include, Gamma (30-80 Hz),
  Beta (13-30 Hz),
   Beta 1 (13-16 Hz),
    Beta 2(16-20 Hz),
   Beta 3 (20-30 Hz),
  SMR(13-15 Hz),
  Alpha(8-13 Hz),
  Mu (9-11 Hz),
  Theta(4-8 Hz),
 and Delta (1-4 Hz).

\[
P_{\text{band},i} = \sum_{k=f_{\text{low}}}^{f_{\text{high}}} PSD_{i,w}(k) 
\]
where the Power Spectrum Density  is obtained by normalizing the Power Spectrum using the product of the sampling frequency 
and the frame size  
\[
PSD_{i,w}(k) = \frac{|F_{i,w}(k)|^2}{fs \cdot \text{frame}}
\] and 
\[
F_{i,w}(k) = \text{FFT}\{X_{i,w}\} ,
X_{i,w} \text{ denote the } w^\text{th} \text{ window of the } i^\text{th} \text{ channel's signal}\]



\paragraph{Root Mean Square (RMS)} For each channel $x_i$, the RMS is computed with:
\[
    \text{RMS} = \sqrt{\frac{1}{T}\sum_{j=1}^{T} x_{i, j}^2}
\]


in reality, the signal is often divided into windows of overlapping signals before the RMS is computed, and thus the dimension of the final RMS signal is dependent on the number of windows (or patches) that are eventually selected.

Note that RMS can be generalized into a few other metrics. Specifically, RMS is the norm of \textbf{Simple Square Integral} $\text{SII} = \sum_{j=1}^{T} x_{i, j}^2$, and can be converted to a slightly more complex form named \textbf{V-Order} as
$
V = \left( \frac{1}{T} \sum_{j=1}^{T} x_{i,j}^v \right)^{\frac{1}{v}}
$.
% is xxx. 
The later is derived from a mathematical model of EMG signal generation, aims to estimate the muscle contraction force. 
% It is mathematically represented as follows, where \(x_{i,j}\) denotes the amplitude at the \(j^{th}\) timestamp of the \(i^{th}\) channel:
%\[
%V = \left( \frac{1}{N} \sum_{j=1}^{N} x_{i,j}^v \right)^{\frac{1}{v}}
%\]
Here, when \(v\) = 2, this feature equals to the RMS.


%\paragraph{ n-th Temporal Moments}
%\[
%TMn_i =\lvert \frac{1}{N} \sum_{j=1}^{N} (x_{i,j} )^n \rvert
%\]

% \paragraph{Log Detector} (LOG) utilizes the logarithm of EMG signal amplitudes to estimate muscle contraction forces. It is defined as:
%\[
%LOG = e^{\left( \frac{1}{N} \sum_{j=1}^{N} \log(|x_{i,j}|) \right)}
%\]



\paragraph{Waveform Length (WL)} For each channel $x_i$:
\[
    \text{WL} = \sum_{j=1}^{T-1}\left|x_{i, j+1}-x_{i, j}\right|
\]
Note that Willison Amplitude (wAMP) is the above, with a requirement that the difference $\left|x_{i, j+1}-x_{i, j}\right|$ is greater than a threshold.
This feature is defined as the amount of times that the
change in EMG signal amplitude exceeds a threshold; it is
an indicator of the firing of motor unit action potentials
and is thus a surrogate metric for the level of muscle contraction.

% Note that temporal moment (TM) is also an one-to-one mapping of this function; Log Detector (LD) might be an one-to-one mapping of this function. [CHECK]

Also, the Average Amplitude Change (AAC), also known in literature as the Difference Absolute Mean Value (DAMV), is a feature that quantifies the average magnitude of amplitude changes between consecutive samples in a signal. It is nearly equivalent to WL
feature, except that wavelength is averaged:
$AAC_i = \frac{1}{N-1} \sum_{j=1}^{N-1} \left| x_{i,j+1} - x_{i,j} \right|
$.

% where:
% \begin{itemize}
%     \item \(N\) is the total number of timestamps in the \(i^{th}\) channel,
%     \item \(\left| x_{i,j+1} - x_{i,j} \right|\) represents the absolute difference in amplitude between consecutive samples.
% \end{itemize}

% This formulation emphasizes the average amplitude change per sample, providing insights into the signal's overall amplitude variability and is indicative of the muscular activity's intensity and characteristics.



Another feature relating to WL is the Maximum Fractal Length (MFL) for each channel is defined as:

\[
MFL_i = \log_{10} \left( \sqrt{\sum_{j=1}^{N-1} (x_{i,j+1} - x_{i,j})^2 } \right)
\]

MFL has different definition, checking this..........

% where:
% \begin{itemize}
%     \item $N$ is the total number of timestamps in the $i^{th}$ channel.
%     \item The term $(x_{i,j+1} - x_{i,j})^2$ computes the squared difference between consecutive timestamps, capturing the incremental changes in the signal.
%     \item The square root of the sum of these squared differences quantifies the overall 'path length' traversed by the signal in the $i^{th}$ channel, adjusted for the scale of the differences.
%     \item The logarithm base 10 ($\log_{10}$) transformation normalizes this path length, facilitating the comparison of fractal complexity across different channels or signals.
% \end{itemize}

This formulation enables the analysis of fractal characteristics and complexity in multi-channel signals, offering insights into their inherent patterns and behaviors.



\paragraph{Zero Crossing (ZC)} For each channel $x_i$:
\[
    \text{ZC} = \sum_{j=1}^{T-1} \left[ \left|x_{i, j+1}-x_{i, j}\right| \geq \text { threshold }\right], \text{ where } \left(x_{i, j} \times x_{i, j+1}\right) < 0
\]
% %[1993]-"A New Strategy for Multifunction Myoelectric Control" (3) for reference

% The Zero Crossing (ZC) feature for electromyography (EMG) data quantifies the frequency content of the waveform by counting the number of times the signal crosses zero within a specified window. To reduce noise-induced zero crossings, a threshold is applied. Given two consecutive samples $X_k$ and $X_{k+1}$, the zero crossing count, $ZC$, is incremented if the following conditions are met:

% \begin{enumerate}
%     \item $X_k > 0$ and $X_{k+1} < 0$, or $X_k < 0$ and $X_{k+1} > 0$, indicating a change in the sign of the waveform, and
%     \item The absolute difference between the two samples $|X_k - X_{k+1}| \geq 0.01 \, V$, ensuring that the change is significant and not due to noise.
% \end{enumerate}


Consider a multichannel EMG signal represented by a sequence of samples $\{x_{i,j}\}$, where $i$ indexes the channel and $j$ indexes the timestamp within each channel. The zero crossing count $ZC_i$ for the $i^{th}$ channel within a window can be mathematically defined as:

\[
ZC_i = \sum_{j=1}^{N-1} \mathbb{1}\left\{ (x_{i,j} \cdot x_{i,j+1} < 0) \, \text{and} \, |x_{i,j} - x_{i,j+1}| \geq \text{Threshold} \right\}
\]

% Given a sequence of EMG signal samples $\{X_k\}$, where $k$ indexes the sample in the sequence, the zero crossing count $ZC$ within a window can be mathematically defined as:

% \[
% ZC = \sum_{k=1}^{N-1} \mathbb{1}\left\{ (X_k \cdot X_{k+1} < 0) \, \text{and} \, |X_k - X_{k+1}| \geq \text{Threshold} \right\}
% \]

where $N$ is the total number of samples within the window, $\mathbb{1}\{\cdot\}$ is the indicator function that evaluates to 1 if its argument is true and 0 otherwise, and the Threshold is established based on the system noise level and gain to reduce the impact of noise-induced zero crossings.

\paragraph{New Zero Crossing (ZC)} ( seems intersting and might be relevant)

% https://ieeexplore.ieee.org/document/8951119

% \[
% fZC(x_{i,j}, x_{i,j+1}) = 
% \begin{cases} 
% 1, & \text{if } (x_{i,j} > T \text{ and } x_{i,j+1} < T) \text{ or } (x_{i,j} < T \text{ and } x_{i,j+1} > T), \\
% 0, & \text{otherwise}.
% \end{cases}
% \]
\[
ZC_i = \sum_{j=1}^{N-1} \mathbb{1}\{ ((x_{i,j} > T \text{ and } x_{i,j+1} < T) \text{ or } (x_{i,j} < T \text{ and } x_{i,j+1} > T))
\]

The threshold \(T\) for identifying significant zero crossings is determined from the resting state samples as:

\[
T = 4 \times \left( \frac{1}{10} \sum_{i=1}^{10} x_{i} \right),
\]

where \(x_{i}\) represents the amplitude of samples in the resting state, and the factor 4 is used to adjust the threshold based on experimental observations.






% \paragraph{Slope Sign Change (SSC)} For each channel $x_i$, we compute the second-order difference between consecutive timestamps:
% \[
%     \text{SSC} = 
% \]

%  Slope Sign Changes -A feature which may provide
% another measure of frequency content is the number of times
% the slope of the waveform changes sign. Once again a suitable
% threshold must be chosen to reduce noise induced slope sign
% changes.
% Given three consecutive samples, Xk-l, Xk and Xk+l, the
% slope sign change count, SC, is incremented if

%https://pubmed.ncbi.nlm.nih.gov/8468080/ the paper with the original definition for ssc
% The Slope Sign Change (SSC) is a feature that counts the number of times the slope of a signal waveform changes its sign, indicating a reversal in the direction of the signal's trend. This feature is a measure of the signal's frequency content. 
% % and is used to identify points of interest within a signal, such as the onset of muscle contractions in EMG analysis.

% Given a signal represented by a sequence of samples $\{X_1, X_2, \ldots, X_n\}$, the SSC is calculated by examining three consecutive samples at a time $(X_{k-1}, X_k, X_{k+1})$. The count of SSC, is incremented under the following conditions:

% \begin{equation}
% SCC = \sum_{k=2}^{n-1} \left\{
%     \begin{array}{ll}
%         1 & \text{if } (X_k > X_{k-1} \text{ AND } X_k > X_{k+1}) \\
%           & \text{OR } (X_k < X_{k-1} \text{ AND } X_k < X_{k+1}) \\
%           & \text{AND } (\left|X_k - X_{k+1}\right| \geq \text{threshold} \\
%           & \text{OR } \left|X_k - X_{k-1}\right| \geq \text{threshold}),
%     \end{array}
% \right.
% \end{equation}

% where the \textit{threshold} is a predetermined value set to minimize the influence of noise. This threshold ensures that only significant changes in the signal's slope are considered, reducing the likelihood of noise-induced slope sign changes being counted.



% The Slope Sign Change (SSC) for the $i^{th}$ channel is computed as:

% \[
% SSC_i = \sum_{j=2}^{N-1} \mathbb{1}\left\{ \left( (x_{i,j} > x_{i,j-1} \, \text{AND} \, x_{i,j} > x_{i,j+1}) \, \text{OR} \, (x_{i,j} < x_{i,j-1} \, \text{AND} \, x_{i,j} < x_{i,j+1}) \right) \, \text{AND} \, \left( |x_{i,j} - x_{i,j+1}| \geq \text{threshold} \, \text{OR} \, |x_{i,j} - x_{i,j-1}| \geq \text{threshold} \right) \right\}
% \]

% where $N$ is the total number of timestamps within the window for each channel, $\mathbb{1}\{\cdot\}$ is the indicator function that evaluates to 1 if its argument is true and 0 otherwise, and the \textit{threshold} is a predetermined value set to minimize the influence of noise on the slope sign change detection.


\paragraph{Slope Sign Change (SSC)}
 Given a signal sequence $\{x_{i,j}\}$ with $i$ indexing the channel and $j$ indexing the timestamp, the Slope Sign Change (SSC) for the $i^{th}$ channel, $SSC_i$, can be defined as:

\[
SSC_i = \sum_{j=2}^{N-1} \mathbb{1}\left\{ \left[ (x_{i,j} - x_{i,j-1})(x_{i,j} - x_{i,j+1}) < 0 \right] \land \left[ \max\left( |x_{i,j} - x_{i,j+1}|, |x_{i,j} - x_{i,j-1}| \right) \geq \text{threshold} \right] \right\}
\]

where $\mathbb{1}\{\cdot\}$ is the indicator function, $N$ is the number of timestamps in each channel, and \textit{threshold} reduces noise influence.







\paragraph{Interquantile Range (IQR)} We consider the variability and distribution of the signal from the quantile perspective: % https://link.springer.com/article/10.1007/s41133-019-0020-7
\[
 IQR_{i,w} = Q_{75}(X_{i,w}) - Q_{25}(X_{i,w}),
\]
25 quantile == $1/4$
IQR for each window in the signal is calculated as the difference between the 75th and 25th percentiles of the samples within that window.

Similar properties include Myopulse Percentage Rate (MPR), enhanced mean absolute value (EMAV)


\paragraph{Teager-Kaiser Energy Operator (LTKEO)}

%https://www.sciencedirect.com/science/article/pii/S0045790617303932
% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7886279



% https://ieeexplore.ieee.org/stamp/stamp.jsp?tp=&arnumber=7886279 this is the link for LKEO
The non-linear TKEO measures instantaneous energy changes of signals composed of a
single time-varying frequency. The proposed feature utilizes
the logarithm of the summation of the TKEO operator in each
analysis window as a nonlinear representation of EMG energy
from each channel.

\begin{equation}
LTKEO_{i} = \log\left( \sum_{j=1}^{N-2} \Psi(x_{i,j}) \right) = \log\left( \sum_{j=1}^{N-2} x_{i,j}^2 - x_{i,j-1} \cdot x_{i,j+1} \right)
\end{equation}

Here, $\Psi(x_{i,j})$ denotes the TKEO of the sample at the $j^{th}$ timestamp of the $i^{th}$ channel, and $N$ represents the total number of timestamps within the analysis window for that channel. The application of the logarithm to the sum of TKEO values across each analysis window provides a powerful representation of the EMG energy for each channel.


% NEO variance:
% Non-linear Energy operator algorithm was made to de-noise electrical neuronal signals. The main
% purpose of NEO is to improve the SNR. If the amplitude of the signal is constant, or zero, the output of
% the NEO is zero: if the amplitude of the signal is drastically changed and has a high peak, the Neo will
% go to the highest value. The NEO applied to a signal x[n] is given by:


This is similarly important in EEG as the Mean Teager Energy (MTE) measure. 

% https://link.springer.com/article/10.1007/s10916-014-0018-0\ link for MTE
The Mean Teager Energy (MTE) is a feature commonly employed in EEG signal analysis to quantify the energy of the signal within a specific window. Defined for the $i^{th}$ channel of an EEG signal, the MTE over a window ending at the $k^{th}$ sample is given by:

\begin{equation}
MTE_{i,k} = \frac{1}{N} \sum_{j=k-N+3}^{k} \left( x_{i,j-1}^2 - x_{i,j-1} \cdot x_{i,j-2} \right)
\end{equation}





\subsubsection{Distance-related}

\subsection{Cross-channel feature}


\paragraph{Global Field Power} GFP constitutes a reference-independent measure of response strength. Mathematically, GFP is the standard deviation of all electrodes at a given time.



\paragraph{Global dissimilarity (DISS)}

Global dissimilarity (DISS) is an index of configuration differences between two electric fields, independent of their strength. 
This parameter equals the square root of the mean of the squared differences between the potentials measured at each electrode (versus the average reference), each of which is first scaled to unitary strength by dividing by the instantaneous GFP.


\paragraph{Phase Locking Value} 

Given two signal channels, let $\phi_{i,w}(k)$ and $\phi_{j,w}(k)$ represent the phase of the $k$th frequency component within the $w$th window of channels $i$ and $j$, respectively. The Phase-Locking Value (PLV) between these two channels over a window $w$ is defined as:

\begin{equation}
PLV_{i,j,w} = \left| \frac{1}{K} \sum_{k=1}^{K} e^{i(\phi_{i,w}(k) - \phi_{j,w}(k))} \right|,
\end{equation}

where:
\begin{itemize}
    \item $K$ is the total number of frequency components considered within the window.
    \item $e^{i(\phi_{i,w}(k) - \phi_{j,w}(k))}$ represents the complex exponential of the phase difference between the $k$th frequency component of channels $i$ and $j$ within the window $w$.
\end{itemize}    

The absolute value $\left| \cdot \right|$ quantifies the degree of phase synchronization, with values closer to 1 indicating higher synchronization and values closer to 0 indicating lower synchronization.


There are many cross-channel features to study the connectivity/causality/correlation between different channels, they are based on the MAR model:

\paragraph{Directed Transfer Function }

Directed Transfer Function (DTF)
The DTF measures the causal influence of channel $x_j$
  on channel $x_i$
  at frequency $f$, based on a multivariate autoregressive (MVAR) model. It is defined as:
  \[\text{DTF}_{j\rightarrow i}^{2}(f) = \frac{\left|H_{ij}(f)\right|^{2}}{\sum_{m=1}^{k}\left|H_{im}(f)\right|^{2}}
\]

$H_{ij}(f)$ represents the element of the transfer matrix 
H(f) from the MVAR model, indicating the influence from channel $x_j$
 to channel 
$x_i$ at frequency 
$f$.
The normalization ensures that DTF values are between 0 and 1.

\paragraph{Partial Directed Coherence}
\[
P_{ij}(f) = \frac{A_{ij}(f)}{\sqrt{a_{j}^{*}(f)a_{j}(f)}}
\]

==> text/exp_v1.tex <==

\section{Experimental Results}

\input{tables/synthetic_table}

% \paragraph{Experimental setups} 
We perform experiments to demonstrate that based on the proposed function modeling framework, \ours~can be a robust alternative approach for pre-training and learning on time series:
\begin{itemize}[noitemsep,leftmargin=*]
    \item We pre-train \ours~on synthetic datasets of autocorrelated sinusoids and fractional Brownian motion (fBm), and validate its advantage over other pre-training methods on feature regression tasks.
    \item We show that by prompt tuning a pre-trained \ours~on real-world tasks, we obtain decent performance with only $\textless 1\%$ new parameters trained.
    \item By training and tuning \ours~in a task-specific way, we achieve comparable or favorable performance across xxx tasks, showing its potential and possibility.
\end{itemize}

\subsection{Synthetic validation: A feature regression task}

\paragraph{Datasets} We build two synthetic datasets with AR components in frequency and time spaces.

\underline{\smash{(1) Superposition of autocorrelated sinusoids.}} We extend previous synthetic datasets based on sinusoids \citep{yoon2019time,das2023decoder}, and build a new synthetic dataset of sinusoids with AR components in the frequency space. 
Specifically, we sample the set of $\{f_i\}_{i=1}^{20}$ based on five random AR(10) processes.
% The constructed data follows \cite{}
% builds additional complexity on top of previous works \citep{some-other-previous-works} that use sine waves, following intuition from neuroscience research. 
%Specifically, the constructed data can be written as:
%\[
% S(t) = \sum_{N} s_i(t) = \sum_{N} a_i \sin (2 \pi f_i t + p_i) + e_k, \text{ where }e_k \sim \mathcal{N}(0, 1)
% \]
% where the frequency components $f_i$ follow an AR(1) process {\color{blue} re-check here and fill in details}, 
We generate amplitude following the $a_i = 1/f_i$ frequency distribution and uniformly sample the phase $p_i \in (0, 2\pi]$.
%\[
%f_k = c_k + \sum_{i=1}^{p} w_i * f_{k-i} \quad \text{{\color{blue} Think about if the other components should be written here this way}}
%\]
% Experimentally, we randomly initialize five different AR processes, and build $N=20$ as the total amount of sine waves. 
% The stochasticity of the generated signal mainly comes from the randomness of the combination of sampled frequencies.
%This design is grounded, as many biosignal studies and others select sine waves as basis of their signals as operators \citep{surana2020koopman}. % and other koopman operator works
We randomly initialize the process {\color{blue} XXX} times. 

% \paragraph{Datasets: fractional Brownian motion (fBm)}
\underline{\smash{(2) Fractional Brownian motion (fBm).}}
We build the next-smoothness prediction task using generated fractional Brownian motion (fBm), which is a generalization of the classical Brownian motion with interdependent increments across time. The constructed data are as follows:
\[
S_H(t):=\frac{1}{\Gamma\left(H+\frac{1}{2}\right)}\left(\int_{-\infty}^0\left[(t-s)^{H-1 / 2}-(-s)^{H-1 / 2}\right] d B(s)+\int_0^t(t-s)^{H-1 / 2} d B(s)\right),
\]
where $\Gamma$ is the Gamma function, the integrator $B$ is the ordinary Brownian process, and $H \in (0, 1)$ is the Hurst parameter. We simulate the process using the Cholesky's Method \citep{dieker2003spectral} with $O(n^3)$ complexity. We remove the signal with abnormal values due to simulation instability (around 0.5\% of all data).

The fBM process has zero expectations across time,  stationary increments, and $1/f^{H+0.5}$ spectral density. Thus, when $H$ varies, the simulated data have short-range or long-range dependency that covers a broad range of data including traffic or stock \citep{rivero2016new}. 

\paragraph{Results on feature regression} We show ...


\subsection{In-context generalization when pre-trained on synthetic functions}

% In this section, we show that, \ours~when pretrained on synthetic datasets with frequency and time functional autoregressive components, demonstrates impressive in-context generalization ability.

% {\color{blue} The following is going to be greatly simplified (appendix-ified).}

% \paragraph{Building synthetic datasets with proper autoregressive components} 

% REF: https://proceedings.neurips.cc/paper_files/paper/2019/file/c9efe5f26cd17ba6216bbe2a7d26d490-Paper.pdf 

% REF: https://arxiv.org/pdf/2108.07799 This is perfect!

% REF: https://proceedings.neurips.cc/paper_files/paper/2022/file/0a9747136d411fb83f0cf81820d44afb-Paper-Datasets_and_Benchmarks.pdf

% Ref this paper as well: https://datasets-benchmarks-proceedings.neurips.cc/paper_files/paper/2021/file/ec5decca5ed3d6b8079e2e7e7bacc9f2-Paper-round1.pdf

% To model the stochasticity in biosignals, specifically, the factors that are unknown to researchers due to the complexity of biological systems, we propose the following two datasets to train transformers to characterize the stochasticity of the system.
% Specifically, we ask the following question: How much can a transformer learn data-dependent information that is beyond distribution-dependent information?

% \paragraph{Stochastic superposition of sine waves}

We build two types of synthetic datasets with autoregressive components on frequency and time space:

\paragraph{Pre-training and validation on synthetic datasets}

% In order to understand the effect and potentials of \ours, we first design a task of reconstruction to understand the capacity of our models.

As shown in Table~\ref{tab:synthetic}, we first validate \ours~performance on synthetic datasets when pretraining them on synthetic datasets. 
As shown in presented results, in comparison to the common next-period prediction task and masked autoencoding task, \ours~is a better pretraining framework.
Our model learns better representation, as indicated by the reconstruction task, regression task, and imputation tasks.
The autoregressive modeling framework provided by \ours~is critical to properly represent the property of the continuous function of time series.


\paragraph{In-context generalization on real-world datasets}

When pretraining on the provided synthetic dataset, our model provides state-of-the-art zero-shot performance. Following previous works \citep{wu2022timesnet}, we perform experiments on classification, imputation, anomaly detection, and forecasting tasks. We show that our model, when comparing against other pre-training methods, demonstrate robust performance, showing its potential on being the foundation model of time series.


\subsection{Training \ours~on real-world datasets}

To show that \ours~is a generalizable framework, we perform experiments as shown in Table~\ref{tab:tasks}.

% \input{tables/task_table}

\paragraph{Experimental Setup} We initialize the weights with a synthetic data pretrained version. Then we perform fine-tuning on the real world dataset, which retrains the transformer with a newly initialized classifier.


\paragraph{Results}

We obtain results on classification, imputation, anomaly detection tasks. We show that \ours~achieves state-of-the-art performance on many tasks.

\input{tables/realworld_table}


\paragraph{Visualizations} To better understand (1) how \ours~encode timeseries into the latent space; (2) the quality of data reconstruction, we plot visualizations.

\subsection{Ablation experiments}

We show that the autoregressive components and the construction of time series sentences are the keys to the success of \ours~. To show this, we perform ablations experiments and change multiple encoder architectures.


\paragraph{Changing the length of TS sentence} Changing the length of the constructed time series sentence. Expectation: Increasing total number would improve performance, but it reaches certain plateau (or scaling law?).


\paragraph{Changing the type of encoders} We have three types of encoders: 1D-Residual blocks, TimeBlocks \cite{wu2022timesnet}, and MLP \cite{nie2022time,liu2022seeing}. We show in Table~\ref{tab:encoder-ablation}, consistently, adding the autoregressive component improves the performance, regardless of the encoder architecture.

\paragraph{Verifying the effectiveness of autoregressive components}
The constructed time series sentence is beyond just providing data augmentation.

\input{tables/ablation_table}


\begin{figure}[t!]
  \centering
  \includegraphics[width=\textwidth,trim={0 10cm 0 10cm},clip]{imgs/visualization_fig_plan.jpg}
  \caption{\textit{Visualizations}. (A) Task-specific visualizations of data. (B) Understanding the effective components in data through sentences of time series. (C) Autoregressive data generation process.}
\end{figure}

\paragraph{Understanding the effective component in data}
One critical advantage of \ours~is that, by constructing timeseries sentence, we can quickly edit our model, and understand the raw component of data. Specifically:
\begin{itemize}
    \item Which component is important in your data, frequency or time?
    \item To which extent (sampling rate, frequency range)?
    \item Which channel is important?
\end{itemize}
Ideally, this section can have some additional visualizations.



==> text/intro_v1.tex <==
\section{Introduction}


Recent advances in large language models (LLMs)
demonstrate the advantage of large-scale pre-training, providing a generalizable way for modeling complex systems \citep{radford2019language}.
At the core of state-of-the-art LLMs is the next-token prediction task \citep{achiam2023gpt}, where each data sample (sentence) is segmented into tokens (words), and the next word is predicted based on the previous words using the transformer architecture 
% (Figure~\ref{fig:overview}(B)) 
\citep{vaswani2017attention}.
By completing samples of sentences based on partial information in an autoregressive (AR) way, LLMs build generalizable data representations that can be rapidly adapted to new datasets and tasks \citep{brown2020language}.

Many works in time series analysis mimic the transformer-based modeling approaches in language by building sequences from samples through segmenting time series into periods of time points (Figure~\ref{fig:overview}(A) \citep{nie2022time,liu2022seeing,zhang2023crossformer}.
However, understanding time series as concatenations of time periods has two issues: (1) it \textit{\textbf{breaks nonlocal functional properties}} like trend or periodicity, and often requires special remedies to compensate for the issues \citep{zhou2022fedformer}; (2) the constructed time periods \textit{\textbf{lack interpretability}}, as the resulting periods are often myopic and hard to analyze unlike common functional bases that are extensively studied in the context of Taylor or Fourier series. 
To compensate for the limitation of segmenting time series, recent works rely on the usage of operators like Fourier neural operators or Koopman operator, but they either require specially engineered coding blocks \citep{liu2023frequency}, or a specific set of predetermined bases that are often not generalizable across datasets \citep{liu2024koopa}.


Motivated by the recent work in computer vision \citep{tian2024visual} that reconsiders the natural sequences for images, in this work,
we take a step back and re-think alternative approaches to build sequences of time series samples by considering them as functions of time.  
Instead of breaking time series into periods, we consider time series samples $\rmS$ as a sampled version of a function $g(t)$ that %, potentially, 
consist of multiple simplified functional components (Figure~\ref{fig:overview}(A)).
% where each of them has a meaning (Figure~\ref{fig:overview}(A)).
% $\{g_1(t), ..., g_N(t)\}$ (Figure~\ref{fig:overview}(B)). 
Instead of mapping the sample to a fixed set of basis like Taylor or Fourier series, 
we isolate the functional components in a data-dependent way by 
% from completely unseen time series, 
building a degradation operator $d_i(\cdot)$ of different intensity levels $i$ to create augmented versions of the same data that contain varying amounts of partial information.
By doing so, we generate an alternative sequence of time series samples, which contains a progressive amount of information from the original sample that is interconnected and eventually greatly simplified.
We train an autoregressive transformer to learn the connection of differently simplified samples, building a knowledge map of different functional components \footnote{For example, in brain decoding tasks, signals often contain cross-frequency coupling where low-frequency components drive the high-frequency components \citep{klimesch2018frequency,donoghue2020parameterizing}.}.
Analogous to the next word prediction task that learns narrative in languages, we denote our method as the Narratives of Time Series (NoTS) because it learns the functional narrative of temporal signals (Figure~\ref{fig:overview}(C)).
% We refer to our methodology as `narratives of time series' (\ours), where we assume that a function as a component of the time series sample should be the proper `word' in time series.

We first justify the construction of an alternative sequence using an intuitive function approximation analysis in Section~\ref{sec:theorysection}.
When learning time series data with transformers, under the universal approximation framework,
we show that learning time series as sequences of periods of time points would cause approximation issues, as performing sampling operation on commonly encountered time series signal processing operators (e.g., differentiation) % or thresholding)
creates discontinuous sequence-to-sequence functions.
Instead, such limitations can be bypassed by forming and learning from the alternative function sequences, as long as either one of the conditions is met: (1) The constructed sequence is expressive, (2) Using an expressive tokenizer \citep{ismailov2023three} before learning with the transformer.
We validate the analytical results experimentally through a feature regression task on synthetic datasets, and show that \ours~significantly outperforms other methods when approximating features with real-world characteristics, showing the potential to approximate a broader class of functions both theoretically and experimentally.


We further validate \ours~in real-world time series datasets in a multitask setting, where we consider performance across 22 real-world datasets consisting of classification, imputation, and anomaly detection tasks.
Across the board, \ours~improves the average performance of other pre-training methods by up to $6\%$,
significantly outperforming next-period prediction, masked autoencoder (MAE), and MAE with Fourier neural operators.
Moreover, we show that \ours~can improve the performance of existing transformer architectures, giving a performance boost when performing dataset-specific pre-training. Interestingly, we present a synthetically pre-trained lightweight model \ourslw,
which can be efficiently adapted to real-world tasks and achieve $82\%$ average performance with only $\textless 1\%$ trainable parameters, showing the potential 
% , significantly outperforming all existing pre-training methods including next-period prediction or masked autoencoders. 
of \ours~on learning generalizable dynamics that can be transferred across datasets and tasks.

The main contributions of this paper are summarized as follows:
\vspace{-2mm}
\begin{itemize}[noitemsep,leftmargin=*]
    \item An alternative approach to form sequences from time series data by considering them as functions of time and isolating functional components with constructed degradation operators.
    \item Analytical results showing that learning time series from the functional perspective allows the approximation of a broader class of functions when compared to learning across periods of time.
    \item A novel transformer-based pre-training framework%\hp{Let's clarify throughout the paper if NoTS refer to a pre-training method, an architecture, or both.} 
    \ours~that progressively reconstruct time series from their degraded variants, and thus learn the interrelationships across functions.
    % components, and reconstructs the original sample in an autoregressive way by considering an increasing amount of functional components in each step.
    \item Experimental results on 2 synthetic and 22 real-world datasets, including 4 different classes of tasks (classification, regression, anomaly detection, and imputation), showing that \ours~significantly outperforms other pre-training methods from next-period predictors to Fourier-informed masked autoencoders, giving a stable performance boost on top of existing architectures. 
    \item A synthetically pre-trained lightweight model \ourslw~that can be efficiently adapted on new datasets and tasks with $\textless 1\%$ parameters trained while maintaining $82\%$ average performance.
\end{itemize}



==> text/method_v1.tex <==
\section{Method: \ours}

% Building on the autoregressive modeling framework, \ours~aims to provide a novel autoregressive method for time series by treating time series samples as functions in time. 

\begin{figure}[t!]
  \centering
  \includegraphics[width=\textwidth]{imgs/NoTS_fig1.png}
  \caption{\textit{Overview of \ours}. (A) Constructing Sentence of time series, and use transformer to predict the next token in an autoregressive manner. (B) To build an architecture that is invariant to the amount of channels and the length of time, we rely on convolutional layer that performs convolution on the time dimension only, with fixed kernels. (C) The transformer has resolution embeddings and positional embeddings. (D) Attention map of autoregressive transformer, where the class token is only attended to the final tokens that try to predict original data.}
\end{figure}

\subsection{Overview: Functional tokenization of timeseries} 

In the time series domain, a multivariate time series sample is represented as $\rmX = [\rvx_1, \rvx_2, ..., \rvx_T] \in \mathbb{R}^{C \times T}$, where $C$ represents the total amount of channels, and $T$ represents the length in time. No matter if it is the channel-independent design, or channel-dependent design, the autoregressive framework produces tokens through cutting time series into different periods of time $L$, which creates tokens $\rvt_i = \operatorname{Tokenizer}([\rvx_i, ..., \rvx_{i+L}])$, and thus $\rmX = [\rvt_1, \rvt_2, ..., \rvt_{T^{\prime}}]$, where $T^{\prime}$ is the length of token sequences after tokenization. Traditional next-period prediction task would directly use the tokenized $\rmX$ and model it as in Equation~\ref{eq:ar_basic}.

Instead of predicting the next period in time, our framework is built on the idea that time series should be a function as a whole that consists of different functional components.
Specifically, $\rmX = [\rvx_1, \rvx_2, ..., \rvx_T]$ is intrinsically a function $g(t)$, where $\rvx_i = g(i)$ is only a product of the sampling process. This view of time series would give better representation of the samples: Consider the same sample under a different sampling operation $\rmX_{\text{undersample}} = [\rvx_2, \rvx_4, ..., \rvx_T]$, building patches of fixed length would result in significantly different tokens, yet they are originated from the same function $g(t)$. 
% , and thus $X$ is an approximated version of $g(t)$. 
% Interestingly, in this view, $[x_{1/2}, x_1, x_{3/2} ..., x_T]$, in the semantic space, is very close to $[x_1, x_2, ..., x_T]$, as long as they are from the same continuous function $g(t)$. 
{\color{blue} Still need better wording and examples here.}

Considering the different aspects of time series, each function $g(t)$ is influenced and controlled by different components. Thus, we treat $g(t) = \operatorname{Combine}([g_1(t), g_2(t), ... g_M(t)])$, where each sample is a combination of $M$ different functional components that are dependent on each other.
Our approach aims to model and learn this relationship. {\color{blue} This paragraph is abundant, and confusing. Also, this $g_i$ as basis is different from the degraded function $g_i$ below. We also don't use any basis because it may be stupid to exhaust them.}

However, it is impossible to exhaust all functions. Thus, our method operates on a `degradation' function $d(\cdot, k)$, that generates degraded version of the sample $\rmX_k = d(\rmX, k)$ as an augmented version of the raw data with only partial information. 
An alternative way to view this is that $g_k(t) = d(g(t), k)$ is a partial form of original function $g(t)$.
Instead of modeling the dependency between periods of time within $\rmX$, we treat $\rmX$ as one complete function $g(t)$, and model the autoregressive relationship between the generated $g_i(t)$ and $g(t)$:
\[
p\left(\rmX_1, \rmX_2, \ldots, \rmX \right)=\prod_{k=1}^K p\left(\rmX_k \mid \rmX_1, \rmX_2, \ldots, \rmX_{k-1}\right), \text{ where } \rmX_K = \rmX
\]
or in the function view:
\begin{equation}
\label{eq:ours_main_overview}
\begin{aligned}
p\left(g_1(t), g_2(t), \ldots, g_K(t)\right)=\prod_{k=1}^K p\left(g_k(t) \mid g_1(t), g_2(t), \ldots, g_{k-1}(t)\right), \\
\text{ where } K \rightarrow \infty, \quad \rvx_i = g_{\infty}(i) \text{ forms the actual time series under the sampling operation}
\end{aligned}
\end{equation}
Here, $k$ represents the intensity of the degradation, or the amount of information lost during the process. As $k$ grows larger and larger, $\rmX_k$ would converge to the given sample $\rmX$ due to the limit of the sampling operation. The resulting $K$ is the sequence for autoregression.

{\color{blue} Need to simplify the overview, and make it stronger/convincing. Need to figure out a better way to introduce the degradation function.}



\subsection{A working model}

Based on the above framework, we performed the following to build a working model.

\paragraph{Selecting degradation functions} We need to select actual degradation functions for the model to work. The selection is based on two criteria: (1) The constructed autoregressive task is prevalent. It should be logical to deduce $g_i(t)$ based on $[g_1(t), g_2(t), ..., g_{i-1}(t)]$, making it possible to perform inference at the next scale; (2) The constructed $g_i(t)$ should be a `simplified' version of the raw function $g(t)$, containing controllable partial information. 
In this work, inspired by many discussion about frequency and time \citep{liu2023frequency}, we build a model with two degradation functions that simultaneously forms the two autoregressive tasks:
\begin{itemize}[noitemsep,leftmargin=*]
    \item \textit{Next-smoothness prediction:} In the time domain, we construct predictive task of the next smoothness by performing window wrapping that `compresses' or `downsamples' a signal:
\[
    \rmX_k = d_{\text{sm}}(\rmX, k) =  (\rmX * w_k)[n], \text{ where } 
w_k[n] = \begin{cases} 
      1/2p_k, & -p_k \leq n \leq p_k \\
      0, & \text{elsewhere}
      \end{cases}
\]
where $*$ represents discrete convolution performed between given data and a kernel $w_k$. 
{\color{blue} Math needs to be consistent here. (1) Decide $\rmX$ or $g(t)$ to write functions throughout. (2) Index.} Here, we use an averaging kernel of different length $2p_k$ to perform convolution on the raw data, and thus creating time series of different smoothness.
% https://arxiv.org/pdf/2002.12478

    \item \textit{Next-frequency prediction:} In the frequency domain, we construct predictive task of the next frequency. We first transform the time series into the frequency domain using Fourier transform (FFT), perform bandpassing of degrade $k$, and then transform the signal back to the time domain using inverse Fourier transform (iFFT):
\[
\rmX_k = d_{\text{fr}}(\rmX, k) = \operatorname{IFFT} (\operatorname{Bandpass}_i (\operatorname{FFT}(\rmX)))
\]
{\color{blue} Can this be written in a better form?}
\end{itemize}

We simultaneously build the above tasks into our model. The resulting autoregressive tasks of time series allow us to comprehend the time series in both time and frequency, covering a wide range of common tasks in the domain of time series.


\paragraph{Autoregressive modeling of groups of tokens in the latent space}
Ideally, we would want to build different classes of functions in time into a discrete latent space to mimic `words' in language. However, it can be impossible to exhaust all possible basis functions in time. Also, encoding sampled functions with varying length into one same token can be computationally infeasible. {\color{blue} Maybe we can mention the reason in an alternative way.} Thus, we rely on encoder $\mathcal{E}$ and decoder $\mathcal{D}$ to extract the latent representations, which forms groups of tokens for the autoregressive modeling task:
\[
\rmR_k = \mathcal{E}(\rmX_k), \quad \rmX_k^{\prime} = \mathcal{D}(\rmR_k^{\prime})
\]
where each $\rmR_k$ consists of multiple tokens, and $\rmR_k^{\prime}$ are deduced from $\rmR_k$ through an autoregressive transformer with group-masked attention map: 
\[
[\rmR_{2}^{\prime}, ..., \rmR_{K}^{\prime}] = \operatorname{AR-Transformer}([\rmR_{1}, ..., \rmR_{K-1}]), 
\text{ where } 
\operatorname{AttN-mask} = \begin{cases} 
      1, & \text{\color{blue} Group mask.} \\
      -\infty, & \text{elsewhere}
      \end{cases}
\]
% Refer to math from that mask context object detection paper
Thus, the autoregressive predictive task in the latent space becomes:
\[
p\left(\rmR_2, \ldots, \rmR_K\right)=\prod_{k=2}^K p\left(\rmR_k \mid \rmR_1, \rmR_2, \ldots, \rmR_{k-1}\right), \text{ where } \rmR_k = \mathcal{E} (\rmX_k)
\]
\text{\color{blue} This equation looks strange, need to re-check.}


In experimental section, we show that \ours~can flexibly work with different encoder/decoder architectures. \text{\color{blue} Should we be more specific here? Maybe that'd help with clarity.} In all of our experiments, we used a very simple 1D-ResNet encoder block that is channel-independent, to keep the best fidelity of the tokens. We show in ablation experiments that other encoder/decoder architectures work.

% and relied on channel-independent modeling of timeseries in zero-shot applications.

% \subsection{Autoregressive modeling with transformers}

\paragraph{Positional embeddings}

Since transformers are inherently invariant to the order of sequences, it is critical to embed sufficient information about the raw position into the transformer to make sure $\rmR_k$ includes sufficient information about $\rmX_k$. Thus, we add the following embeddings:

\begin{itemize}[noitemsep,leftmargin=*]
    \item \textit{Time embeddings}. We apply rotary positional embedding \citep{su2024roformer} to encode relative sequence position along the temporal dimension.
    \item \textit{Channel embeddings}. We add learnable absolute positional embeddings that encode channel-wise relationship within the transformer.
    \item \textit{Resolution embeddings}. We add learnable absolute embeddings that encode the relative information loss across data sentences of time series. In other words, it encodes information $k$ in function $d(\cdot, k)$ for the two different functions $d$.
\end{itemize}

% we add resolution embeddings and position embeddings (where position embedding includes information about both channel and time in the latent space). Then a transformer is used to perform autoregressive modeling. 

\paragraph{Training objective} 
We perform pre-training to learn meaningful representation about time series using the proposed architecture. The pertaining is an autoregressive reconstruction task that optimizes the following loss function for each sample:
\[
    \mathcal{L} = \sum_{i=2}^{K} \underbrace{\mathcal{L}_{\text{recon}}(X_{i+1}^{\prime}, X_i)}_{\text{AR reconstruction}} + \underbrace{\mathcal{L}_{\text{recon}}(\mathcal{D}(\mathcal{E}(X_K)), X_K)}_{\text{latent consistency term}}
\]
where $\mathcal{L}_{\text{recon}}$ is reconstruction loss, where we use MAE loss across the paper.
The first term AR reconstruction loss minimizes the differences between $X_k$ and reconstructed $X_{k+1}^{\prime}$ for every $k$, except the raw data. 
When considering only the first term, the latent of the raw data $\rmR_K$ would remain un-used throughout the training process. To avoid the distributional shift caused by that, we added a \textit{reconstruction consistency term}, that regularizes the consistency between the latent of the raw data to be able to be reconstructed back.

% The whole architecture aims to optimize the following loss function:

% \paragraph{Spectral loss} To also reconstruct the high-frequency components, we also use spectral loss.

%\paragraph{Latent commitment loss} When only using the previous versions of the loss, the raw data latent is left un-used, and would cause the model to ignore the raw data. To make use of the raw latent, we add a latent commitment loss as well:
%\[
%    \mathcal{L}_{\text{commit.}} = \alpha \sum_{k=1}^{K-1} l(R_k, R_{k+1}^{\prime})
%\]


\subsection{In-context generalization through prompt tuning}

One of the most critical challenges of building a generalizable foundation model for time series is to deal with a dataset with new channel-wise relationships. In this work, we make the following hypothesis: The function in time is transferrable and generalizable, yet channel-wise relationship is new for each dataset, and needs to be learned in-context.
% always face a critical issue about generalizing to new channel relationship.
Thus, when having a pretrained model, we adapt the pretrained model in the following way to perform in-context generalization for timeseries to new datasets and tasks.

{\color{blue} As we do perform training, and the training is not few-shot, I am not 100\% sure in-context learning is the right terminology to be used here. The gist is to train as few as new parameters (only the necessary ones) as possible, and do not update the previously learned parameters at all.}

{\color{blue} Maybe we should rename it as context-aware fine-tuning, prompt tuning, or whatsoever.}
% https://arxiv.org/pdf/2301.00234

% However, this is challenging for time series data. Aside from common reasons such as insufficient amount of data, one critical aspect is because different time series data have different channel-wise dependencies. While continuous relationship may be easy to transfer, different channel-wise dependencies are not easy to be generalized or transferred.

\paragraph{Learning new channel-wise relationship} To learn channel-wise relationship in-context, for each dataset, we perform the following two operations on our pretrained model:
\begin{itemize}
    \item[(1)] Initialize new addable channel tokens.
    \item[(2)] To encourage channel mixing and information exchange across channels, we also add a data embedding layer before applying the encoder $\mathcal{E}$. The data embedding layer is a simple linear layer that encodes on the channel dimension $\mathbb{R}^{C} \rightarrow \mathbb{R}^{C^{\prime}}$. It mixs channel-wise information at an early stage, allowing the transformer to obtain more information about channel-wise relationship in each dataset.
\end{itemize}
We couple the new channel-wise relationship to our pretrained model. The gist is that we do not sacrifice the pretrained model in any way (so it is not normal fine-tuning that creates $N \times M$ models for $N$ tasks and $M$ datasets). Instead, we create $M$ learnable channel heads here, and $N$ learnable task heads later, and use one same model for all of them. 
This is to validate that our model learns general-purpose temporal functions have the capacity to be transferred or generalized.


\paragraph{Learning new tasks in-context} To demonstrate that the model is generalizable across different tasks, we add new task-specific parameters in the following ways: (1) Prompting tokens (classification tokens, the data masking tokens in imputation task, and the forecasting tokens in forecasting task); (2) Linear layers for inference (classification linear layer, anamoly detection linear layer).

{\color{blue} TO-DO: Finalize this subsec after deciding which tasks to include}




==> text/method_v2.tex <==
\section{Method: \ours}

\begin{figure}[t!]
  \centering
  \includegraphics[width=\textwidth]{imgs/NoTS_fig1.png}
  \caption{\textit{Overview of \ours}. (A) Constructing Sentence of time series, and use transformer to predict the next token in an autoregressive manner. (B) To build an architecture that is invariant to the amount of channels and the length of time, we rely on convolutional layer that performs convolution on the time dimension only, with fixed kernels. (C) The transformer has resolution embeddings and positional embeddings. (D) Attention map of autoregressive transformer, where the class token is only attended to the final tokens that try to predict original data.}
\end{figure}

\subsection{The next-function prediction task} 

Instead of predicting the next period in time, our framework is built on the idea that time series should be a function in time that consists of different functional components.
To simplify the assumptions, we consider univariate time series, where each data $\rvs = [..., s_i, ...]$ is intrinsically a function $g(t)$, where $s_i = g(i)$ is a product of the sampling process. 
% Consider the same sample under a different sampling operation $\rmX_{\text{undersample}} = [\rvx_2, \rvx_4, ..., \rvx_T]$, building patches of fixed length would result in significantly different tokens, yet they are originated from the same function $g(t)$. 
% {\color{blue} Still need better wording and examples here.}
Each function $g(t) = \operatorname{Combine}([g_1(t), g_2(t), ... g_M(t)])$ consists of $M$ different functional components that are related to each other. A naive example here would be that each musical instrument has its unique high-frequency and low-frequency sounds that are solely dependent on the instrument type.

To learn the relationships across different functional components, on a high-level, we propose to use autoregressive modeling to learn the following:
\begin{equation}
\label{eq:ours_main_overview_hyp}
p\left(g_1(t), g_2(t), \ldots, g_M(t)\right)=\prod_{m=1}^M p\left(g_m(t) \mid g_1(t), g_2(t), \ldots, g_{m-1}(t)\right)
\end{equation}

% Thus, we treat $g(t) = \operatorname{Combine}([g_1(t), g_2(t), ... g_M(t)])$, where each sample is a combination of $M$ different functional components that are dependent on each other.

% Our approach aims to model and learn this relationship. {\color{blue} This paragraph is abundant, and confusing. Also, this $g_i$ as basis is different from the degraded function $g_i$ below. We also don't use any basis because it may be stupid to exhaust them.}

% This view of time series would intrinsically give a more robust representation of the data when they are sampled from different sampling rates.

While treating time series from the functional perspective might be advantageous for many reasons, practically, we would ask two questions: (1) How to isolate different functional components, as they tend to change across different tasks or datasets? (2) How to determine the direction of the causality, as the relationships may vary across different tasks or datasets?

% However, it is impossible to exhaust all functions. 
To address the above two issues, practically, we propose to construct `degradation' functions $d_k(\cdot)$ of intensity $k$, that generate augmentations of the original function $g(t)$ with varying amounts of partial information. Specifically, it would create $g^{\prime}_k(t) = (d_k \circ g)(t)$, where $g^{\prime}_{k+1}(t)$ contains strictly more or equal amount of information than $g^{\prime}_{k}(t)$ about the original sample $g(t)$. Thus, the new modeling approach becomes the following:
\begin{equation}
\label{eq:ours_main_overview}
\begin{aligned}
& p\left(g^{\prime}_1(t), g^{\prime}_2(t), \ldots, g^{\prime}_K(t)\right)=\prod_{k=1}^K p\left(g^{\prime}_k(t) \mid g^{\prime}_1(t), g^{\prime}_2(t), \ldots, g^{\prime}_{k-1}(t)\right), \\
\text{ where } & K \rightarrow \infty, \quad s_i = g^{\prime}_{\infty}(i) \text{ forms the actual time series $\rvs$ under the sampling operation}
\end{aligned}
\end{equation}
By constructing a degradation function, we can (1) isolate different functional components by selecting different types of degradations, and (2) build a natural autoregressive sequence as the deduced function always contains more information than the previous functions.

% $\rmX_k = d(\rmX, k)$ as an augmented version of the raw data with only partial information. 
% An alternative way to view this is that $g_k(t) = d(g(t), k)$ is a partial form of original function $g(t)$.

% Instead of modeling the dependency between periods of time within $\rmX$, we treat $\rmX$ as one complete function $g(t)$, and model the autoregressive relationship between the generated $g_i(t)$ and $g(t)$:
Practically, as we perform the operations based on a sampled signal $\rvs$, we generate discrete augmentations of $\rvs$ and perform the autoregressive modeling as follows:
\[
p\left(\rvs_1, \rvs_2, \ldots, \rvs_K \right)=\prod_{k=1}^K p\left(\rvs_k \mid \rvs_1, \rvs_2, \ldots, \rvs_{k-1}\right), \text{ where } \rvs_K = \rvs
\]
% Here, $k$ represents the intensity of the degradation, or the amount of information lost during the process. As $k$ grows larger and larger, $\rmX_k$ would converge to the given sample $\rmX$ due to the limit of the sampling operation. The resulting $K$ is the sequence for autoregression.
% {\color{blue} Need to simplify the overview, and make it stronger/convincing. Need to figure out a better way to introduce the degradation function.}
where $\rvs_k = d_k(\rvs)$ for $1 \leq k \leq K-1$.


\subsection{A working model}

Based on the above framework, we construct a model \ours~with the following details.

\paragraph{Local and global smoothing degradation functions} To construct meaningful degradation functions, we rely on convolution operators with kernels containing either local or global properties:
\begin{equation}
\begin{aligned}
    \rvs_k = d_k(\rvs) =  (\rvs * w_k)[n] % \text{ where } 
% w_k[n] = \begin{cases} 
%      1/2p_k, & -p_k \leq n \leq p_k \\
%      0, & \text{elsewhere}
%      \end{cases}
\end{aligned}
\end{equation}
where $*$ represents discrete convolution performed between given signal and a kernel $w_k$. 
\begin{itemize}[noitemsep,leftmargin=*]
    \item \textit{Local smoothing:} For local smoothing, we select a simple averaging kernel of different lengths. Specifically, $w_k[n] = 1/2p_k$ for $-p_k \leq n \leq p_k$ and $w_k[n] = 0$ elsewhere. 
% {\color{blue} Math needs to be consistent here. (1) Decide $\rmX$ or $g(t)$ to write functions throughout. (2) Index.} 
Here, we use an averaging kernel of different length $2p_k$ to perform convolution on the raw data, and thus creating time series of different smoothness.
% https://arxiv.org/pdf/2002.12478
    \item \textit{Global smoothing:} For global smoothing, we construct a low-pass filter with different frequency cutoff values. $w_k[n] = sinc(p_k)$ {\color{blue} fill in details}. We create time series of different frequency components by performing this operation. It is worth noting that the operation is a brick-wall filter in the frequency space.
    % We first transform the time series into the frequency domain using Fourier transform (FFT), perform bandpassing of degrade $k$, and then transform the signal back to the time domain using inverse Fourier transform (iFFT):
% \[
% \rmX_k = d_{\text{fr}}(\rmX, k) = \operatorname{IFFT} (\operatorname{Bandpass}_i (\operatorname{FFT}(\rmX)))
% \]
% {\color{blue} Can this be written in a better form?}
\end{itemize}

By constructing both local and global smoothing degradation functions, the proposed method can simultaneously model autoregressive relationships across different smoothness and frequencies, covering a prevalent range of tasks in both time and frequency. 
%It should be logical to deduce $g_i(t)$ based on $[g_1(t), g_2(t), ..., g_{i-1}(t)]$, making it possible to perform inference at the next scale; (2) The constructed $g_i(t)$ should be a `simplified' version of the raw function $g(t)$, containing controllable partial information. 
% In this work, inspired by many discussion about frequency and time \citep{liu2023frequency}, we build a model with two degradation functions that simultaneously forms the two autoregressive tasks:

% We simultaneously build the above tasks into our model. The resulting autoregressive tasks of time series allow us to comprehend the time series in both time and frequency, covering a wide range of common tasks in the domain of time series.


\paragraph{Autoregressive modeling of groups of tokens in the latent space}
Ideally, we would want to build different classes of temporal functions into a discrete latent space to mimic `words' in language. Practically, it is challenging to do so as time series has varying lengths, and certain samples can have substantial length (e.g. 5000) to be coded as one low-dimensional token.
% Also, encoding sampled functions with varying length into one same token can be computationally infeasible. {\color{blue} Maybe we can mention the reason in an alternative way.}
Thus, in this work, we rely on encoder $\mathcal{E}$ and decoder $\mathcal{D}$ to extract the latent representations, which form groups of tokens for each sample to create the autoregressive modeling task:
\[
\rmR_k = \mathcal{E}(\rvs_k), \quad \rvs_k^{\prime} = \mathcal{D}(\rmR_k^{\prime})
\]
where each $\rmR_k$ consists of multiple tokens with relative position $\Omega_k$, and $\rmR_k^{\prime}$ are deduced from the set of $\rmR_k$ through an autoregressive transformer with group-wise masking on the attention map: 
\[
[\rmR_{2}^{\prime}, ..., \rmR_{K}^{\prime}] = \operatorname{Transformer}([\rmR_{1}, ..., \rmR_{K-1}]), 
\text{ where } 
\operatorname{mask}[\Omega_k] = \begin{cases} 
      0, & \bigcup_{m=1}^{k+1} \Omega_{m} % \text{ till } \Omega_{k+1}%\text{\color{blue} Group mask.} 
      \\
      -\infty, & \text{elsewhere}
      \end{cases}
\]
{\color{blue} Need suggestions on make this index less confusing} where $\Omega_k$ represents the token positions correspond $R_k$.
% Refer to math from that mask context object detection paper
Thus, the autoregressive predictive task in the latent space becomes:
\begin{equation}
p\left(\rmR_2, \ldots, \rmR_K\right)=\prod_{k=2}^K p\left(\rmR_k \mid \rmR_1, \rmR_2, \ldots, \rmR_{k-1}\right)
\end{equation}
% \text{\color{blue} This equation looks strange, need to re-check.}


Experimentally, we implement $\mathcal{E}$ and $\mathcal{D}$ with 
% flexibly work with different encoder/decoder architectures. \text{\color{blue} Should we be more specific here? Maybe that'd help with clarity.} In all of our experiments, we used 
a simple 1D-ResNet encoder/decoder block that is channel-independent, to maintain the fidelity of the tokens. % We show in ablation experiments that other encoder/decoder architectures work.

% and relied on channel-independent modeling of timeseries in zero-shot applications.

% \subsection{Autoregressive modeling with transformers}

\paragraph{Positional embeddings}

Since transformers are inherently invariant to the order of sequences, it is critical to embed sufficient information about the raw position into the transformer to make sure $\rmR_k$ includes sufficient information about samples. Thus, we add the following embeddings:

\begin{itemize}[noitemsep,leftmargin=*]
    \item \textit{Time embeddings}. We apply rotary positional embedding \citep{su2024roformer} to encode relative sequence position along the temporal dimension.
    \item \textit{Channel embeddings}. We add learnable absolute positional embeddings that encode channel-wise relationship within the transformer.
    \item \textit{Resolution embeddings}. We add learnable absolute embeddings that encode the relative information loss across data sentences of time series. In other words, it encodes information $k$ of the degradation function $d_k(\cdot)$.
\end{itemize}

% we add resolution embeddings and position embeddings (where position embedding includes information about both channel and time in the latent space). Then a transformer is used to perform autoregressive modeling. 

\paragraph{Training objective} 
We perform self-supervised autoregressive reconstruction task to learn meaningful representations about time series using the proposed architecture. For an input data $\rmX$, the training optimizes the following loss function for each sample:
\[
    \mathcal{L} = \sum_{k=1}^{K-1} \underbrace{\mathcal{L}_{\text{recon}}(\rmX_{k+1}^{\prime}, \rmX_k)}_{\text{AR reconstruction}} + \underbrace{\mathcal{L}_{\text{recon}}(\mathcal{D}(\mathcal{E}(\rmX_K)), \rmX_K)}_{\text{latent consistency term}}
\]
where $\mathcal{L}_{\text{recon}}$ is the reconstruction loss, where we use MAE loss throughout.
The first AR reconstruction term minimizes the differences between $\rmX_k$ and reconstructed $\rmX_{k+1}^{\prime}$ for every $k$, except the raw data. 
When considering only the first term, the latent of the raw data $\rmR_K$ would remain unused throughout the training process. To avoid the distributional shift caused by that, we added a \textit{latent consistency term}, that regularizes the consistency between the latent of the raw data to be able to be reconstructed back.

\subsection{Context-aware generalization through prompt tuning}
\label{sec:prompt-tuning-method}

One of the most critical challenges of building a generalizable foundation model for time series is to deal with a dataset with new channel-wise relationships. Towards this end, we propose a prompt tuning pipeline based on the following assumptions: The function in time is transferrable and generalizable, yet channel-wise relationship is new for each dataset, and needs to be learned in context.
% always face a critical issue about generalizing to new channel relationship.
Thus, when having a pre-trained model, we adapt the pre-trained model in the following way to perform context-aware generalization for time series to new datasets and tasks.

% {\color{blue} Maybe we should rename it as context-aware fine-tuning, prompt tuning, or whatsoever.}
% https://arxiv.org/pdf/2301.00234

\paragraph{Tuning channel adaptors} To learn channel-wise relationship for each dataset, we perform the following two operations when adapting our pre-trained model on specific datasets:
\begin{itemize}
    \item[(1)] To encourage information exchange across channels, we add a data embedding layer before applying the encoder $\mathcal{E}$. The data embedding layer is a simple linear layer that encodes on the channel dimension $\mathbb{R}^{C} \rightarrow \mathbb{R}^{C^{\prime}}$ to mix channel-wise information at an early stage.
    \item[(2)] We also re-initialize and re-train addable channel tokens for each dataset.
\end{itemize}

\paragraph{Tuning task adaptors} The model is generalizable across different tasks, both generative and discriminative ones. To adapt a pre-trained model on different tasks, we add new task-specific parameters in the following ways: (1) We add prompt tokens to the transformer architecture along with data tokens following the deep VPT plan \citep{jia2022visual}; (2) We also add task-specific linear layers at the end of the transformer for inference.

Combining the two adaptors, the prompt tuning pipeline train $\textless 1\%$ new parameters of the model with frozen weights, giving an efficient learning plan, without having to adjust any weights from the pre-trained model.
% We couple the new channel-wise relationship to our pretrained model. 
Thus, unlike normal full-model fine-tuning regime where one has to create $N \times M$ models for $N$ tasks and $M$ datasets, our model requires only $N$ task adaptors and $M$ channel adaptors that are both light-weight. 
% Instead, we create $M$ learnable channel heads here, and $N$ learnable task heads later, and use one same model for all of them. 
This pipeline can be used to demonstrate if a pre-trained model learns general-purpose temporal functions that can be 
% have the capacity to be
transferred or generalized.

% {\color{blue} TO-DO: Finalize this subsec after deciding which tasks to include}




==> text/relatedworks_wenrui.tex <==
\section{Preliminaries and related works}

\subsection{Preliminaries}
\paragraph{Autoregressive modeling} Popular large language models (LLMs) are famous for being `next token predictors'. 
A sample in the language domain is typically a sentence $X = [\rvx_1, \rvx_2, ..., \rvx_T]$, where each $\rvx_i \in \mathcal{V}$ is a discrete token of `word' from a given vocabulary. The next-token prediction task is about modeling the autoregressive relationship as follows: The probability of obtaining the next token $\rvx_i$ can be deduced by the observed subsequence $[\rvx_1, \rvx_2, ..., \rvx_{i-1}]$. Thus, the probability of obtaining the whole sample can decomposed as the product of a sequence of unidirectional conditional probabilities:
\begin{equation}
\label{eq:ar_basic}
p\left(\rvx_1, \rvx_2, \ldots, \rvx_T\right)=\prod_{i=1}^T p\left(\rvx_i \mid \rvx_1, \rvx_2, \ldots, \rvx_{i-1}\right)
\end{equation}
In practice, the autoregressive relationship is typically learned by a transformer model $p_\theta$ parameterized by $\theta$. Next-token predictors have demonstrated impressive in-context generalization capability, as they can be easily prompted to perform multiple tasks that are unseen during the training process.
% generalizability.

\paragraph{Notations and tokenizers for time series} Time series samples are sequences of data points recorded from different channels.
An univariate time series sample is represented as $\rvs = [s_1, ... s_i, ..., s_T] \in \mathbb{R}^{T}$, where $T$ represents the length of signal in time. A sample normally has many channels, which forms a multivariate time series sample as $\rmS = [\rvs_1, ..., \rvs_j, ..., \rvs_C]^\top = [\rvv_1, ..., \rvv_i, ..., \rvv_T] \in \mathbb{R}^{C \times T}$, where $C$ represents the total amount of channels. Each dataset typically has its unique channel-wise relationships.
% Many works consider the channel-independent design, which processes each channel $\rvx_j$ independently. The other works map all channels in each dataset to a common latent space, and build collective representation for each time point $i$. {\color{blue} Think about best place to put this paragraph.}

% \paragraph{Traditional tokenizers} 
Many time series framework produces tokens through cutting time series into different periods of time with a length of $L$, which creates tokens $\rvx_i = \operatorname{Tokenizer}([\rvv_{iL}, ..., \rvv_{(i+1)L}])$, and thus producing $\rmX = [\rvx_1, \rvx_2, ..., \rvx_{\ceil{T/L}}]$. These types of works map all channels in each dataset to a common latent space, and build collective representation for each time point $i$. Another line of works consider the channel-independent design, which processes each channel $\rvs_j$ independently, and produce tokens based on individual channels, and occasionally allow transformers to learn their interrelationships. Traditional next-period prediction tasks would directly use the tokenized $\rmX$ and model it as in Equation~\ref{eq:ar_basic}. Alternatively, masked autoencoders would perform the masking and then prediction pre-training technique.
% {\color{blue} Think about best place to put above two paragraphs.}

\subsection{Pretraining methods for time series}

% {\color{blue} Maybe Jingyun can help write this subsection?}

Include related works of the following:
\begin{itemize}
    \item \textbf{[FOCUS]} Pretraining methods for time-series. We need to benchmark them.
        \begin{itemize}
               \item\cite{darlow2024damfoundationmodeltime} This work proposes DAM, a foundation model for time series that does forecasting tasks by taking randomly sampled histories and outputs an adjustable
basis composition as a continuous function of time for forecasting to unlimited length of horizons. The basis is constructed using pre-defined sine waves, and they did not patchy things but rather sample discrete time points from both past and future, and do reconstruction by using Huber loss for training.

\item Generative pre-training:

\begin{itemize}



    \item \cite{rasul2024lagllamafoundationmodelsprobabilistic} proposes Lag-Llama which uses a decoder-only transformer architecture. It uniquely employs lags as covariates, which allows it to effectively capture dependencies in time series data. This approach focuses on leveraging historical data points (lags) as inputs to the model, enabling it to generate accurate forecasts based on past trends.

\item \cite{garza2024timegpt1} introduces TimeGPT-1 on the other hand, adopts an encoder-decoder structure with several transformer layers. This design facilitates efficient zero-shot forecasting, allowing the model to generalize well across different types of time series without needing task-specific fine-tuning. The encoder-decoder architecture helps TimeGPT-1 handle complex sequences and dependencies in time series data, making it a versatile and powerful forecasting tool.

\item \cite{liu2024timergenerativepretrainedtransformers},Timer uses a GPT-style architecture. It curated a highly heterogeneous dataset with up to 1 billion time points, unified into a single-series sequence (S3) format. It is pre-trained through next-token prediction and adapted to various downstream tasks. It predicts the next series via autoregression, generates imputations with masked tokens, and performs predictive anomaly detection by forecasting normal series

        \cite{woo2024unifiedtraininguniversaltime} proposes Masked EncOder-based
UnIveRsAl TIme Series Forecasting Transformer
(MOIRAI), which is a novel Transformer architecture designed for universal time series forecasting, overcoming limitations in existing models that assume independent variates or fixed dimensionality. It achieves this by flattening multivariate time series into a single sequence and introducing Any-variate Attention, which uses binary attention biases to differentiate between variates while ensuring permutation equivariance and invariance. MOIRAI also employs a multi-patch size projection layer approach, allowing it to handle a wide range of time series frequencies by adapting patch sizes to the data's frequency, reducing computational costs while maintaining long context lengths.

\item \cite{dong2023simmtmsimplepretrainingframework} found that randomly masking a portion of time points
will seriously distort vital temporal correlations of time series, making the reconstruction task too difficult to guide representation learning. So they proposes SimMTM, which is a pre-training framework for time series modeling that recovers original series from multiple randomly masked versions using neighborhood aggregation. It reconstructs the series by combining point-wise representations based on learned similarities in the series-wise space, guided by both reconstruction and constraint losses. SimMTM excels in fine-tuning, achieving state-of-the-art results in forecasting and classification tasks, even across domain shifts. Its key innovation lies in leveraging manifold learning for effective masked time series modeling.  the original time series by adaptive aggregating multiple masked time series based on series-wise similarities learned contrastively from data.



\item some classic ones: \cite{10.1145/3447548.3467401} TST  follows the standard masked modeling approach, predicting missing time points from the remaining ones. \cite{Yuqietal-2023-PatchTST} proposes PatchTST that improves on this by predicting masked subseries-level patches, capturing local semantics while reducing memory usage.






\end{itemize}


\item Contrastive pre-training:




.


               
        \end{itemize}
        
    \item Works that directly adapt/engineer LLMs for time series.

    \begin{itemize}
        \item \cite{zhou2023fitsallpowergeneraltime}This paper proposes a unified framework that transfers pre-trained parameters from language models (GPT2) to all major time series analysis tasks by freezing the self-attention and feedforward layers, while only training the embedding, normalization, and output layers. The authors show that self-attention functions similarly to PCA, also successfully apply this method to other pre-trained transformers from different backbones(BERT) and modalities(vision)
        \item \cite{jin2024timellmtimeseriesforecasting} This paper proposes TIME-LLM, a framework that reprograms (edit) input time series into text prototypes suitable for LLMs  and augments the input with declarative prompts that describes the tasks, context,as well as the basic statistics of the dataset to guide reasoning, without altering the pre-trained backbone model . TIME-LLM excels in mainstream forecasting tasks, particularly in few-shot and zero-shot scenarios, while maintaining high reprogramming efficiency. 

        \item \cite{liu2024calfaligningllmstime}

        \item \cite{cao2024tempopromptbasedgenerativepretrained} proposes TEMPO, fine tune pre-trained GPT2
        \cite{liu2024autotimesautoregressivetimeseries} proposes AutoTimes, a framework that repurposes large language models (LLMs) for time series forecasting by introducing "in-context forecasting," where time series are treated as prompts, extending the prediction context. AutoTimes integrates textual timestamps as position embeddings and achieves state-of-the-art performance with minimal parameters and faster training/inference.
        \cite{xue2023promptcastnewpromptbasedlearning} proposes PromptCast turns numerical inputs and outputs into prompts, framing forecasting as sentence-to-sentence conversion to leverage language models for direct forecasting.

        \cite{sun2024testtextprototypealigned} proposes TEST, which emphasizes that we should align the time series better to the token embedding space of the LLM, 




        
        
    \end{itemize}
    \item Other works and architectures.
    \item \cite{dooley2023forecastpfnsyntheticallytrainedzeroshotforecasting} This work proposes ForecastPFN, the
first zero-shot forecasting model trained purely on a novel synthetic data distribution. ForecastPFN is a prior-data fitted network, trained to approximate Bayesian
inference, which can make predictions on a new time series dataset in a single
forward pass.

    \item \cite{dong2024timesiampretrainingframeworksiamese}
proposes Timesiam, which is trained by reconstructing masked current series from randomly sampled past observations. The same encoder is used for these inputs, where the samples in the past served as key and value, and the samples from the current serve as query where the cross attention gave us the reconstructed output.







\end{itemize}

==> text/theory_v1.tex <==
% \section{\ours~is more robust under UA theory}
\section{\ours~can approximate functions better}
% \section{What types of Bio-features are difficult for Time-series Transformers?}

In this section, we provide a theoretical analysis to show that \ours~can approximate a broader class of functions under the universal approximation framework. 
% We show that certain discontinuous functions that are commonly met in timeseries analysis cannot be approximated by a normal transformer encoder, but can be approximated by \ours.

{\color{blue} Need to make sure that notations throughout in this section is consistent with previous section. Currently, this section is a standalone version.}

\subsection{Preliminaries}

\paragraph{Transformers} 
The transformer network is the stack of transformer blocks. Consider a sequence-to-sequence function from $\mathbb{R}^{d \times n}$ to $\mathbb{R}^{d \times n}$. The transformer blocks consist of:
\begin{equation}
\begin{aligned}
\operatorname{Attn}(\boldsymbol{X}) & =\boldsymbol{X}+\sum_{i=1}^h \boldsymbol{W}_O^i \boldsymbol{W}_V^i \boldsymbol{X} \cdot \sigma\left[\left(\boldsymbol{W}_K^i \boldsymbol{X}\right)^T \boldsymbol{W}_Q^i \boldsymbol{X}\right] \\
\mathrm{FF}(\boldsymbol{X}) & =\operatorname{Attn}(\boldsymbol{X})+\boldsymbol{W}_2 \cdot \operatorname{ReLU}\left(\boldsymbol{W}_1 \cdot \operatorname{Attn}(\boldsymbol{X})+\boldsymbol{b}_1 \mathbf{1}_n^T\right)+\boldsymbol{b}_2 \mathbf{1}_n^T
% \mathrm{FF}(\boldsymbol{X}) & =\operatorname{Attn}(\boldsymbol{X})+\boldsymbol{W}_2 \cdot \operatorname{ReLU}\left(\boldsymbol{W}_1 \cdot \operatorname{Attn}(\boldsymbol{X})\right)
\end{aligned}
\end{equation}
where $\boldsymbol{W}_O^i \in \mathbb{R}^{d \times m}, \boldsymbol{W}_V^i, \boldsymbol{W}_K^i, \boldsymbol{W}_O^i \in \mathbb{R}^{m \times d}, \boldsymbol{W}_2 \in \mathbb{R}^{d \times r}, \boldsymbol{W}_1 \in \mathbb{R}^{r \times d}$.
We denote $t^{h, m, r}: \mathbb{R}^{d \times n} \rightarrow \mathbb{R}^{d \times n}$ as a Transformer block with an attention layer with $h$ heads of size $m$, and a feed-forward layer with $r$ hidden nodes. Thus, we define the transformer as:
\[
\mathcal{T}^{h, m, r}:=\left\{g: \mathbb{R}^{d \times n} \rightarrow \mathbb{R}^{d \times n} \mid g \text { is a composition of Transformer blocks } t^{h, m, r} \text {, s }\right\} .
\]
Similarly, transformer with absolute positional embedding is:
\[
\mathcal{T}_{\mathrm{P}}^{h, m, r}:=\left\{g_{\mathrm{P}}(\boldsymbol{X})=g(\boldsymbol{X}+\boldsymbol{E}) \mid g \in \mathcal{T}^{h, m, r} \text { and } \boldsymbol{E} \in \mathbb{R}^{d \times n}\right\}
\]

\paragraph{Universal Approximator (UA)} 
Previous research has demonstrated what types of transformer networks are UAs of sequence-to-sequence functions. Specifically, given two functions $f_1, f_2: \mathbb{R}^{d \times n} \rightarrow \mathbb{R}^{d \times n}$, for $1 \leq p<\infty$, we define a distance between them as
$$
\mathrm{d}_p\left(f_1, f_2\right):=\left(\int\left\|f_1(\boldsymbol{X})-f_2(\boldsymbol{X})\right\|_p^p d \boldsymbol{X}\right)^{1 / p}
$$
being UA means that for any given $f_1 \in \mathcal{F}_{}$, let $1 \leq p<\infty$ and $\epsilon>0$, there exists a network $f_2$, such that $\mathrm{d}_p(f_1, f_2) \leq \epsilon$.


\textbf{Theorem 1 (\cite{yun2019transformers}).} 
Let $1 \leq p<\infty$ and $\epsilon>0$, then for any given $f \in \mathcal{F}_{\mathrm{PE}}$ which consists of all continuous permutation equivariant functions with compact support, there exists a Transformer network $g \in \mathcal{T}^{2,1,4}$, such that $\mathrm{d}_p(f, g) \leq \epsilon$, so that transformer is UA for $\mathcal{F}_{\mathrm{PE}}$.

\textbf{Theorem 2 (\cite{yun2019transformers}).}
Let $1 \leq p<\infty$ and $\epsilon>0$, then for any given $f \in \mathcal{F}_{\mathrm{CD}}$ which consists of all
continuous functions with compact support, there exists a Transformer network $g \in \mathcal{T}_{\mathrm{P}}^{2,1,4}$ such that we have $\mathrm{d}_p(f, g) \leq \epsilon$, so transformer with APE is UA for $\mathcal{F}_{\mathrm{CD}}$.

\textbf{Theorem 3 (\cite{luo2022your}).} Transformers with relative positional embedding (RPE) are not UA for $\mathcal{F}_{\mathrm{CD}}$.

While UA theory is typically or traditionally used for understanding continuous functions, more recently, it is recently also used to understand discontinuous functions, and it is shown that relatively easy network can approximate discontinuous functions:

\textbf{Theorem 4 (\cite{ismailov2023three}).} A three-layer neural network can approximate any arbitrary (including discontinuous) functions $\mathbb{I}^d \rightarrow \mathbb{R}$, where $\mathbb{I}$ means $[0, 1]$. \textbf{Make this theorem more formal.}


\cite{ismayilova2023kolmogorov} also showed similar results. This is an important result, such that many real-world systems, physical ones or physiological ones, are often not continuous.

\subsection{The challenge of approximating certain bio-features}

\textbf{Key argument: Although transformers can approximate continuous seq-2-seq functions, for time series, many common operations done on the continuous functions in time, are discontinuous operations.}

% \textbf{Would-be-cool-to-have argument: Although transformers can approximate continuous seq-2-seq functions, for time series, even continuous operations done on the continuous functions in time, can become discontinuous after the sampling operation and thus not approximatable.}

Using transformers to learn timeseries is more challenging than one may expect. Specifically, timeseries typically consider input as function of time $h_1(t)$, and aims to map it to another function of time $h_2(t)$, and using transformer to learn such mapping is considering if function $g(x)$ can map $h_1(t)$ to $h_2(t)$, given a specific sampling of timepoints within. Without loss of generality, we discuss single channel time series (input $X$ of shape $1 \times N$, where $d=1$).

\paragraph{Differentiations cannot be approximated} Many biosignal contain phase operations, and the transition of phase typically rely on differentiations. However, it is well known that differentiation as a mapping function is not continuous, and it is easy to prove that they are not approximatable via transformers, with or without positional embedding.

\paragraph{$\#$1 Example} Consider temporal function $h_1(t)$ and its resulting input $X$ after the sampling operation; as well as temporal function $h_2(t)$ and its resulting expected output as $Y$. A simple example for differentiations is as follows:
\[
\begin{aligned}
 \text{Input: } h_1(t) = \frac{\sin(Mt)}{M} \quad & \xrightarrow[]{sampling} \quad X = [\frac{\sin(Mt_1)}{M}, \frac{\sin(Mt_2)}{M}, ..., \frac{\sin(Mt_N)}{M}] \\
 \text{Output: } h_2(t) = \cos(Mt) \quad & \xrightarrow[]{sampling} \quad Y = [ \cos(Mt_1), \cos(Mt_2), ..., \cos(Mt_N)]
\end{aligned}
\]
We treat the mapping of differentiation as function $g_M: X \rightarrow Y$, and aim to argue if a transformer function $g$ can approximate it.

In this case, $M \rightarrow \infty$ will give $X \rightarrow \mathbf{0}$. Thus, $g(\boldsymbol{X})$ converges to $c \mathbf{1}_n^{\top}$ when without positional embedding, and converges to $c \mathbf{1}_n^{\top} + \mathbf{v}$ when with fixed (absolute) positional embedding. \textbf{Proof of convergence in Appendix}.
% https://arxiv.org/pdf/2107.12530 -- Infinite stacking of transformer layers, it does have specific requirements for the activation functions.
However, one can easily shown that, when the sampling operation is not perfectly periodic (aliasing), e.g. $t_i = i\pi/M$, the function approximation will give an error:
\[
\text{Given } t_{i+1} - t_i = \frac{\pi}{M} \text{ and } N>1, \Rightarrow  \sup _{\boldsymbol{X} \in \mathcal{D}}\left\|\tilde{g}_M(\boldsymbol{X})-g(\boldsymbol{X})\right\|_F \geq \frac{N}{2}
\]
% the phase of $h_2(t) = \cos(Mx)$ constantly change, there exists a bound given specific sampling strategy.
Consider two inputs $t_i^{(1)} = \frac{i\pi}{M}$ and $t_i^{(2)} = \frac{(i+0.5)\pi}{M}$, consider the output of $g$ being $c \mathbf{1}_n^{\top} + \mathbf{v}$, the above is apparently true.


\paragraph{Data-dependent thresholding cannot be approximated} 

\textbf{Wait, what is the necessary condition here, just piecewise discontinuity or something else as well?}

Thresholding is very commonly used in time series analysis. For thresholding, one needs to set a concrete thresholding value, and one common operation is to perform data-dependent thresholding based on the distribution (global property) of time series (global thresholding). For example, setting the $30\%$ lowest value of a time series to zero. In this case, we can also easily prove that they are not approximatable.

% While Piecewise functions cannot be approximated within constant bound.

\paragraph{$\#$2 Example} 
% 0, 0, 1, 1
% 0, 0.1, 1, 1
% sudden change in the second entry? esp, if the threshold value is the average of the sequence?
% 
Given $n>2, d$ and $\mathcal{D} \subseteq \mathbb{R}^{n \times d}$, assume that the all-zero matrix $\mathbf{0} \in \mathcal{D}$. For any $M>0$, there exists a function $\tilde{g}_M: \mathcal{D} \rightarrow \mathbb{R}^{n \times d}$, such that
\[
 \sup _{\boldsymbol{X} \in \mathcal{D}}\left\|\tilde{g}_M(\boldsymbol{X})-g(\boldsymbol{X})\right\|_F>MN
\]
holds for any $g \in \Omega_{\mathrm{RPE}}^{H, d_H, r}$, where $H, d_H, r \in \mathbb{N}^*$.

Consider $\tilde{g}_M: \boldsymbol{X} \mapsto(-M, -M, \cdots, M, M)^{\top}$, as the sorted quantile of the distribution. Consider $g(\mathbf{0})=c \mathbf{1}_n^{\top}$, then we have:
\[
 \left\|\tilde{g}_M(\mathbf{0})-g(\mathbf{0})\right\|_F^2 = N(M-c)^2+N(-M-c)^2 > N^2 M^2 \Rightarrow \sup _{\boldsymbol{X} \in \mathcal{D}}\left\|\tilde{g}_M(\boldsymbol{X})-g(\boldsymbol{X})\right\|_F > NM
\]





% A seq to seq permutation equivariant function that is discontinuous: Let \( \mathbf{V} = \{\mathbf{v}_1, \mathbf{v}_2, \ldots, \mathbf{v}_n\} \) be a sequence of vectors in \( \mathbb{R}^d \). Define a function \( h: \mathbb{R}^d \rightarrow \mathbb{R}^d \) as follows:

% For each vector \( \mathbf{v}_i \) in \( \mathbf{V} \),
% \[
% h(\mathbf{v}_i) = 
% \begin{cases} 
% \mathbf{M} & \text{if } ||\mathbf{v}_i||_2 > \theta, \\
% \mathbf{-M} & \text{if } ||\mathbf{v}_i||_2 \leq \theta,
% \end{cases}
% \]

% where
%\begin{itemize}
%    \item \( ||\mathbf{v}_i||_2 \) denotes the Euclidean norm of \( \mathbf{v}_i \),
%    \item \( \theta \) is a predefined threshold,
%    \item \( \mathbf{M} \)  is a predefined vector in \( \mathbb{R}^d \).
%\end{itemize}

% This function is discontinuous due to the abrupt change in output when the norm of \( \mathbf{v}_i \) crosses \( \theta \), and it is permutation-equivariant because the operation applied to each vector \( \mathbf{v}_i \) is independent of its position in the sequence \( \mathbf{V} \).

%\paragraph{Phase functions (differentiation) as bio-feature extractors}
% https://math.stackexchange.com/questions/3364463/is-differentiation-as-a-map-discontinuous

% Consider a very simple case, where we want to map $f_1(x) = sin(x)$ to $f_2(x) = cos(x)$ using a neural network. We know that $f_1(x)^2 + f_2(x)^2 = 1$, which result in 


The results can be intuitively understood as such: Attention $\operatorname{Attn}$ gives arbitrarily small shifts when the input gives arbitrarily small shifts (it converges) under XXX activation function, and thus the remaining MLP that operates on each individual tokens (context ids, as in below paper).
% https://openreview.net/pdf?id=nJnky5K944
Or to say, it is critical to form contextual mapping, which is shown to be critical in other analysis. That is to say, without meaningful individual tokens, the global property cannot be successfully modeled.


\subsection{Resolving the challenge with properly constructed autoregressive task}

We show that, \ours~can address the above issue if a proper sentence of timeseries can be constructed. Specifically, we show that (1) if the constructed sentence is as long as the timeseries sequence; (2) if the constructed sentence can form a proper mapping between sentence $i$ to output value $i$, \ours~can approximate, at least the above two negative examples.


In this case, we are replacing $\boldsymbol{X}$ to sentence of time series, which is $\boldsymbol{X}_{\text{sent}} = [\boldsymbol{X_1}, \boldsymbol{X_2}, ..., \boldsymbol{X_N}]$. 

\paragraph{Diff} \textbf{It is important to consider the fact that in previous X, the dimension is $n \times 1$ ($d=1c$), and in this case, $d=lc$, where $l$ is the length of signal.}

\textbf{Argument 1} We rely on the fact that an encoder $\mathcal{E}$ with decent complexity can approximate any arbitrary function from $\mathbb{I}^d \rightarrow \mathbb{R}$. Passing the constructed $\boldsymbol{X}_{\text{sent}} = [\boldsymbol{X_1}, \boldsymbol{X_2}, ..., \boldsymbol{X_N}]$ into $\mathcal{E}$, one obtain $[\boldsymbol{R}_1, \boldsymbol{R}_2, ..., \boldsymbol{R}_N]$.

\textbf{Argument 2} As long as the resulting $[\boldsymbol{R}_1, \boldsymbol{R}_2, ..., \boldsymbol{R}_N]$ can form a continuous sequence to sequence function to the expected output $[y_1, y_2, ..., y_N]$, the constructed sentence of time series can approximate it, based on the previous results of \cite{yun2019transformers}.

Note that while the existing result assumes the constructed sentence would require length of $T$, in reality, as long as the constructed sentence represents sufficient information for a period $L$ of time, one only need to craft a sentence of length $T/L$. \textbf{Make this a formal argument}

\textbf{$\# 1$ Example solution} 
\textbf{Actually, d as an identity function can be directly used to approximate this}
The differentiation problem, or phase transition problem, can simply be resolved by crafting a sentence of phase transition.
Specifically, consider constructing $X_k = \sin(Mt + k)/M$, and as long as the encoder has the capacity to select the proper item from the constructed sentence $X_k$, the proper $R_k$ can be formed. Thus, the latter mapping from the sentence of $R_k$ to $Y$ becomes a trivial one-to-one mapping.
% \textbf{Two scenarios in this case $c=1$: $\mathbb{R}^{n \times l} \rightarrow \mathbb{R}^{n \times l}$, or $\mathbb{R}^{n \times l} \rightarrow \mathbb{R}^{1 \times l}$, the difference may be critical -- for the latter case, if the constructed length is greater than the predicted length, it is definitely true, no matter if it is continuous or discontinuous function}.

\textbf{$\# 2$ Example solution} Similarly, xxx


% \subsection{Understand the implication from the perspective of contextual mapping}

% The intuition can be understood from contextual mapping, a key step in proving the transformers are universal approximations \cite{yun2019transformers}. 

% Contextual mapping has restrictions for the embedding space, specifically, it requires the input tokens to be different from each other when their meaning is different. However, when cutting time series into patches, or pixels, this requirement cannot be fulfilled, and thus it does not have the capacity to approximate continuous function in time. \textbf{Need more proper and careful understanding of the original proof to make this correct.}

% Issue: The autoregressive construction must not converge to zero, otherwise it is impossible to form the argument. Does that mean a non-zero embedding layer that forms proper contextual mapping?



==> text/theory_v2.tex <==
% \section{\ours~is more robust under UA theory}
\section{An intuitive example: Approximating functions}
% \section{What types of Bio-features are difficult for Time-series Transformers?}

In this section, we provide a theoretical analysis to show that constructing augmentations of time series in the function form, with their global properties maintained, allows transformer to approximate a broader class of functions under the universal approximation framework.
{\color{blue} If possible, I want to shrink the text of this section by 1/3 page and include a visualization}


\begin{wrapfigure}{r}{0.5\textwidth}
  \begin{center}
    \includegraphics[width=0.48\textwidth]{imgs/NoTS_fig2_sketch.png}
  \end{center}
  \caption{Sketch, how does it look?}
\end{wrapfigure}


\paragraph{Preliminaries: Transformers and Universal Approximators (UA)}
% most recent work on this topic: https://arxiv.org/pdf/2305.12205
% UA implies universal classification: https://papers.nips.cc/paper/2020/file/786ab8c4d7ee758f80d57e65582e609d-Paper.pdf (shrinking the space makes approximation easier)
% \paragraph{Transformers and Universal Approximators (UA)} 
The universal approximation framework considers the feasibility or existence of neural networks that can be used to approximate different types of functions with arbitrarily small error. 
Consider a transformer network $f_2$ and an arbitrary function $f_1$, where $f_2, f_1: \mathbb{R}^{n \times d} \rightarrow \mathbb{R}^{n \times d}$ both are sequence-to-sequence functions. We define a distance between $f_2$ and $f_1$ as:
$$
\mathrm{d}_p\left(f_1, f_2\right):=\left(\int\left\|f_1(\boldsymbol{X})-f_2(\boldsymbol{X})\right\|_p^p d \boldsymbol{X}\right)^{1 / p} % , \text{where } 1 \leq p<\infty
$$
being UA means that for any given $f_1 \in \mathcal{F}_{}$, let $1 \leq p<\infty$ and $\epsilon>0$, there exists a network $f_2$, such that $\mathrm{d}_p(f_1, f_2) \leq \epsilon$.


Previous research have demonstrated that transformer networks (detailed definitions in Appendix) are UAs of all continuous sequence-to-sequence functions \citep{yun2019transformers}.
Interestingly, \cite{luo2022your} shows that changing the absolute positional embedding to relative positional embedding would impair the approximation ability of transformers.


\subsection{The challenge of approximating certain time series operations}

One would quickly discover the unique challenges of approximating time series operations with a transformer when posing the approximation question in the function space. 

We consider a time series $\rvs$ sampled from function $g(t)$.
% Using transformers to learn timeseries is more challenging than one may expect. 
% Under a fixed sampling rate, we consider 
Operations on time series maps input function $g(t)$ to a target function $h(t)$, and then sampling operation with a fixed sampling rate is performed to form the resulting sequence-to-sequence function $f_1$, which is approximated by transformer network $f_2$.
Without loss of generality, we form transformer input $\rmX$ by treating each time point individually (such that $n=T, d=1$).


\paragraph{Example: The case of differentiation} Consider an input $g_M(t) = \frac{\sin(Mt)}{M}$ and its product function after differentiation $h(t) = \cos(Mt)$, and a sampling sequence of $[t_1, t_2, ..., t_T]$. Under the same sampling rate, we consider a random value of $t_1 \in \mathbb{R}$. This operation forms a sequence-to-sequence function $f_1: \mathbb{R}^{T \times 1} \rightarrow \mathbb{R}^{T \times 1}$. Consider the case $M \rightarrow \infty$, we have the following:
\[
\text{Given } t_{i+1} - t_i = \frac{\pi}{M} \text{ and } T>1, \quad \sup _{\boldsymbol{X} \in \mathcal{D}}\left\|f_1(\boldsymbol{X})-f_2(\boldsymbol{X})\right\|_F \geq \frac{T}{2}
\]
Proof sketch: As $M \rightarrow \infty$, input sample $\boldsymbol{X} \rightarrow \mathbf{0}$. We show that $f_2(\boldsymbol{X})$ converges to $c \mathbf{1}_n^{\top}$ when without positional embedding, and converges to $c \mathbf{1}_n^{\top} + \mathbf{v}$ when with fixed (absolute) positional embedding. The resulting target, which is a sampled version of $h(t)$, will be impossible to be approximated. {\color{blue} appendix to write, this can be a lemma}

While in functional space, the above operation on sinusoids can be written as simple phase transition (addition on $t_1$) and multiplication, after the sampling process, it becomes a discontinuous differentiation mapping that is not approximatable by transformers, with or without positional embeddings.

\subsection{Resolving the challenge by modeling sample sequences}

In this section, we show how the above approximation issue can be addressed by constructing and modeling sequences of time series with transformer, when using a % Kolmogorov’s mapping
three-layer
neural network as a tokenizer.
% can address the above issue if a proper sentence of timeseries can be constructed. Specifically, we show that (1) if the constructed sentence is as long as the timeseries sequence; (2) if the constructed sentence can form a proper mapping between sentence $i$ to output value $i$, \ours~can approximate, at least the above two negative examples.
Our results rely on the theorem from \cite{ismailov2023three}, which shows that a % Kolmogorov’s mapping 
three-layer neural network 
%(which can be implemented as a three-layer MLP) 
can be implemented exactly as any arbitrary (continuous or discontinuous) function $f: \mathbb{I} ^n\to \mathbb{R}$, where $n>1$ is a natural number and $\mathbb{I}$ is a compact interval $[0, 1]$.


\paragraph{Solution to differentiation} Consider the example of differentiation, we first construct a sequence of time series from $\rmX$ to a sequence as:
\[
\rmX_{\text{seq}} = [\rmX_1, \rmX_2, ..., \rmX_n], \text{where } \rmX_i \text{ is sampled from } \frac{1+\sin(Mt)+i\delta/n}{M} \text{ \color{blue} [re-check bound]}
\]
% build n*d --> (n) n*d --> (n) d
where $\delta \in (0, M-2]$ is an arbitrary number that distinguishes $\rmX_i$. In this case, we know the existence of a Kolmogorov’s mapping neural network $\mathcal{E}$ that could be used to create certain
$\rmR_i = \mathcal{E}(\rmX_i) \in \mathbb{R}^{d}$ (e.g. $\rmR_i = Mt_i$) that forms $\rmR = [\rmR_1, \rmR_2, ..., \rmR_n]^{\top} \in \mathbb{R}^{n \times d}$, of which there exists a continuous sequence-to-sequence function to the desired target.
Thus, we can guarantee that a transformer that learns on the sequence of constructed samples $\rmR$ can approximate the target output, as it is an universal approximator of any continuous sequence-to-sequence function \cite{yun2019transformers}.

{\color{blue} consider the possibility of generalizing this to a theorem, or at least proposition, noting the accessibility through (1) Ultra expressive encoder; (2) Ultra suitable TS sentence}



% Our result is relevant to the fact that 
Note that, in general, universal approximation only proves existence instead of attainability, and our analysis requires assumptions including the use of specific encoder $\mathcal{E}$, and the minimal length $n$ of the constructed sequence. In later sections, we show that experimentally, our proposed method works without such strong assumptions.

% would require length of $T$, in reality, as long as the constructed sentence represents sufficient information for a period $L$ of time, one only need to craft a sentence of length $T/L$. \textbf{Make this a formal argument}



